Reparameterized Policy Learning for Multimodal Trajectory Optimization

We investigate the challenge of parametrizing policies for reinforcement learning (RL) in high-dimensional continuous action spaces. Our objective is to develop a multimodal policy that overcomes limitations inherent in the commonly-used Gaussian parameterization. To achieve this, we propose a principled framework that models the continuous RL policy as a generative model of optimal trajectories. By conditioning the policy on a latent variable, we derive a novel variational bound as the optimization objective, which promotes exploration of the environment. We then present a practical model-based RL method, called Reparameterized Policy Gradient (RPG), which leverages the multimodal policy parameterization and learned world model to achieve strong exploration capabilities and high data efficiency. Empirical results demonstrate that our method can help agents evade local optima in tasks with dense rewards and solve challenging sparse-reward environments by incorporating an object-centric intrinsic reward. Our method consistently outperforms previous approaches across a range of tasks. Code and supplementary materials are available on the project page https://haosulab.github.io/RPG/

==> draft_5_27.tex <==
Probability is the way go from local to global. Model is the communication from the world to the agent.

\begin{itemize}
    \item Gradient descent works pretty well in practice, but it can not do global exploration. 
    \item It would be nice if we can combine gradient-based optimization method and sampling based approach. 
    \item Adding local noise is not a good choice because of the discontinuities and local minima.
    \item Better structured parameterization. View policy family as a differential map from the random noises into a manifold.
    \item Sample globally with structures; decouple exploration and exploitation; the reason to introduce variational inference. Argument: (sub-)optimal should exhibit low-dimensional structures. 
    \item Able to handle discontinuities and was able to find global optimum more consistently.
\end{itemize}

Advantages of our approach
\begin{itemize}
    \item Potential to search for global optimization (unify search and optimization).
    \item Potential to avoid integration over discontinuous region. (differentaibility and policy gradient)
    \item Consistent hierarchical exploration (hierarchical RL).
    \item Works better than Gaussian based exploration in dynamic environment (exploration issue).
    \item Environment modeling and reusable skill learning.. (representation and skill learning)
\end{itemize}

Disadvantage (defense)
\begin{itemize}
    \item Our goal is not to find a single sub-optimal solution, but to enumerate all possible good solution.
    \item Structure constraints may lead to sub-optimal solution but usually optimal solution will have structures and if we can provide good prior, it will be good. At least better than adding Gaussian noise..
\end{itemize}

Contributions
\begin{itemize}
    \item a structured variational policy learning framework and its connection to maximum entropy learning/EM/VAE;
    \item with differentiable physics, and the extended policy gradient theorem under mild conditions (its implicit benefits on not continuous environments).
    \item applications in skill learning.
\end{itemize}

\paragraph{Statistic} mean field approximation; method of steepest descent or \href{https://physics.stackexchange.com/questions/14639/how-is-the-saddle-point-approximation-used-in-physics}{saddle-point method}; \hza{} optimal trajetory should be simple to analyze? can we get value functions through laplacian transformation?  

\hza{Can we view the decreasing of the alpha entropy as optimizing $\log p_{\gamma}(O)$ by decreasing decreasing the entropy?}


\subsubsection{Value network, discounted return and generalized advantage estimation}

\todo{}: the transition probabilities of the environment is cancelled no matter if the environment is deterministic or not.

\todo{}: before back-propogate the gradient from $s_{t+1}$ to $s_t$, one need multiply the gradient of state $s_{t+1}$ by $\lambda \gamma$ in GAE.

We can view the value network as a truncated gradient helper, and we only need that for random variables. 


% Proof: removing reward and with only the discriminator, we can ensure that trajectories fall within the continuous region. Then prove that for each continuous domain and some proper policy parameterization, gradient descent will converge to the global optimum of the posterior estimation.

\citet{dekkers1991global}

==> figure/graphical_model.tex <==

\begin{figure}
    \centering
    
\begin{subfigure}[t]{0.4\textwidth}
\centering
\begin{tikzpicture}[main/.style = {draw, circle}, node distance=2cm] 
\node[deterministic] (s1) {$s_t$}; 
\node[deterministic] (s2) [right of= s1]{$s_{t+1}$}; 
\node[random] (z2) [below of= s1]{$z_{t}$}; 
\node[random](z1) [left of=z2] {$z_{t-1}$}; 
\node[deterministic](a1) [below of=z2] {$a_t$}; 
\node[deterministic] (R) [below of= a1]{$R_t$}; 
\node (t) [below of=z1]{$\theta$};
\draw [arrow] (s1) -- (s2);
\draw [arrow] (z1) -- (z2);
\draw [arrow] (s1) -- (z2);
\draw [arrow] (z2) -- (a1);
\draw [arrow] (a1) -- (s2);
\draw [arrow] (t) -- (z2);
\draw [->] (s1.west) to [out=240, in=120] (a1.west);
\draw [arrow] (a1) -- (R);
\draw [->] (s1.east) to [out=-40, in=50] (R.east);
\end{tikzpicture} 
\caption{Policy gradient.}
\label{fig:pg}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.4\textwidth}
\centering
\begin{tikzpicture}[main/.style = {draw, circle}, node distance=2cm] 
\node[deterministic] (s1) {$s_t$}; 
\node[deterministic] (s2) [right of= s1]{$s_{t+1}$}; 
\node[random] (z2) [below of= s1]{$z_{t}$}; 
\node[random](z1) [left of=z2] {$z_{t-1}$}; 
\node[deterministic](a1) [below of=z2] {$a_t$}; 
\node[deterministic] (R) [below of= a1]{$R_t$}; 
\node (t) [below of=z1]{$\theta$};
\draw [arrow] (s1) -- (s2);
\draw [arrow] (z1) -- (z2);
\draw [arrow] (s1) -- (z2);
\draw [arrow] (z2) -- (a1);
\draw [arrow] (a1) -- (s2);
\draw [arrow] (t) -- (a1);
\draw [arrow] (t) -- (z2);
\draw [->] (s1.west) to [out=240, in=120] (a1.west);
\draw [arrow] (a1) -- (R);
\draw [->] (s1.east) to [out=-40, in=50] (R.east);
\end{tikzpicture} 
\caption{RPG}
\label{fig:rpg}
\end{subfigure}
\caption{Graphics Model. \ref{fig:pg} is the original policy gradient. while $\ref{fig:rpg}$ is what we study.}
\label{fig:graphics_model}
\end{figure}


==> notes/hrl.tex <==
The major problem is that any method that includes search to encourage exploration will face the problem of learning offline policies, while differentiable physics can only work for online optimization. We have to assume that we can always train low-level policy network until convergence easily. 

Then what should we do? The obvious option is using state space as subgoal directly, for which we only train diffskill like feasibilty predictor or value networks. The issue of this approach is that it may require us to be able to sample for the whole state space, which is usually not true because we do not know it before or it is high-dimensional (for example, have some random noises).

On the other hand, it's much simpler to sample from a sub-space. However, in this case, we can not only learn a goal-conditioned policy —— as it may suffer from the skill-chaining issue, and we can not do whole space planning, as we do not have the Markovian state. We can, of course, still do planning by learning the pseudo model.

We have to let the networks learn a mapping from subgoal trajectories into low-level actions? Let value $V(s, g)$ to represent the value that we have, and let's assume that we have train $V$ well from the online-data. Then given any $g$ and subgoal $o$, we can train $\pi(s, o, g)$ for one stage based on the value $V$. We sample $o$ for efficient exploration (where we have to train the feasibility predictor in an online manner).
This is a simple hierarchical framework. The only issue is that it does not maintain an explicit frontier set and connect it to unknown.

==> text/experiments_old.tex <==
\section{Applications}
\subsection{State-based Exploration}
% We introduce latent variable $z_2$ sampled from $q_\phi(z_2|s)$, then, in this case, we will need to add the term $-\log q_\phi(z_2|s)$

We add the intrinsic reward $-\log p(s)$ to encourage state coverage, which can be implemented with a state-action VAE. 

\hrule

The problem with reconstructing the observation is that we should not rely on its original metric space but should be as accurate as possible in the end.

We do not have to unify the state coverage into our framework. After all, it is neither simple nor natural.

What's the problem with DFS-based (single-modality search)? This seems a very deep question, and we can't answer it now. At least its story is far from the maximum-entropy exploration.

\subsection{Latent Goal Learning}
Instead of using VAE to learn a feature space of the goal, we can directly build a task-driven goal representation. Like HER, we relabel the state's latent with a trajectory's ending or future state and ask the agent to minimize its distance to its target.

\subsection{Hierarchical RL}
The hierarchical policy is related to state representation.

\subsection{Multi-modal Optimization}


\section{Experiment}
% \textbf{Goals}
% \begin{itemize}
%     \item Our approach can benefit from the gradient descent and learn faster than sampling-based methods in certain cases (high-dimensional trajectory optimization). [need carefully designed experiments.]
%     \item Our methods can help gradients to explore global minima and model multi-modality trajectories. [Continuous bandit and maze are enough.]
%     \item Get rid of the discontinuities and chaos.
%     \item Applications in rigid and soft body manipulation.
%     \item Discovery hidden structures [roughly finished].
% \end{itemize}

% \textbf{Experiments}
% All experiments should have some. 
% \begin{itemize}
%     \item Navigation problems with local minima. In this case, the policy gradient converges slower for low batch size, and the gradient gets stuck.
%     \item Discontinuous environment (throw balls with collisions).
%     \item Inverted pendulum gradually increases the discount factor.
%     \item Demonstrate the multiple-trajectories found [roughly ok now in maze environments.]
%     \item Soft body push/pinch [in case we need it].
% \end{itemize}

% What we truly need to prove by experiments
% \begin{itemize}
%     \item Multimodality policy is useful for exploration. 
%     \item Outperforms either zeroth-order or first-order methods.
%     \item Has a really powerful ability to represent complex modalities. While modeling high-level modalities, how we should handle the local uncertainties/very sharp locals.
%     \item Differences of the latent space. Why we need a discrete component and how we handle infinite modalities?
%     \item Large scale experiments.
% \end{itemize}


% \subsection{Experiment outlines}

% Implementation: 
% 1). PPO version RPG that supports hierarchical structures (sample $z$ every $k$ steps). 2). TD-MPC, and revise its MPC to RPG policy. 

% \subsubsection{Tasks}
% \begin{itemize}
%     \item RL environments in ManiSkill 
%     \item Bandit and 2D Move Tasks.
%     \item Differentiable physics environments [the current is enough.]
% \end{itemize}


% \subsubsection{Questions}
% \textbf{\textcolor{red}{Multi-modality policy is necessary for exploration}}
% Baseline: Gaussian head policies. 1) SAC with maximum entropy RL; 2) PPO with RND.
% Showing that under RND, we have a better exploration than PPO on 2D move. 

% \textbf{\textcolor{red}{Importance of the cycle-consistency}} Compare with Option-critic; More like a baseline by removing the mutual information terms.

% \textbf{Why do we need model the trajectories directly?} Compare with learning multi-modality head:normalizing flow, the diffusion models or SQL. This shows the importance of the temporal modeling, amortized inference. Importance of the consistent exploration and low-dimensional sample space. \textcolor{red}{The baseline is necessary.}

% \textbf{Experiments on Maniskill} Multi-ball pick; Tool use (stack a ball and a box);

% \textbf{Ablation of differentiable physics [outperform zeroth order method]}
% Under the model-based learning setting, converges faster than TD-MPC. The same offline Q learning setup while we use function approximation with multi-modalities for learning the policy.


% Remaining questions [for ablations]
% \begin{itemize}
%     \item \textbf{Latent distributions} Why do we have a categorical distribution? Can we use Gaussian or diffusion model?
%     \item \textbf{Structure of trajectory optimization}(Less important) Evaluate the trajectory modeling part (of using different forms of trajectory encoder/decoder). This is more suitable to be studied in the imitation learning task first.
% \end{itemize}

\subsection{Numerical Experiments}

\subsubsection{Environment and evaluation}
 In this section, we investigate the following questions: 1) Whether our method is more efficient for trajectory optimization than gradient-free algorithms; 2) Whether our method can search over the large solution space and avoid local optima that might trap a single-modality policy. % this is a good question to add later, we need a traj distribution visualization plot to answer this question % 3) Whether our method can properly model the trajectory posterior distribution given optimal through variational policy learning. We also demonstrate how different properties of the environment affect our method's performance. 
 
We design the following environments to answer these questions. \textbf{Bandit 1 and 2}: Our bandit problems in Figure~\ref{fig:num_exps}-(1) and Figure~\ref{fig:num_exps}-(2) have a $1$d action space and a non-convex reward landscape. We initialize our policy as a Gaussian centralized around $0$ with its scale barely touching the right mode of reward. The reward function of \textit{Bandit 2} contains an additional discontinuous point. 
\textbf{Move 1 and 2}: An agent moves in a 2D environment for a fixed number of steps and receives a reward according to its terminal position. The terminal reward landscape contains $4$ Gaussian peaks (deeper color = higher reward), as shown in Figure~\ref{fig:num_exps}-(3) and (4). The agent is initialized at the center. Note that the reward of \textit{Move 1} near the initialization point is constant, so the agent receives a non-zero gradient only if it arrives at a position closer to one of the four Gaussian peaks. \textbf{Move 3}: The terminal reward shown in Figure~\ref{fig:num_exps}-(5). There is one obstacle consisting of three white circles. When an agent runs into an obstacle, it will bounce off (continuous collision detection~\citep{hu2019difftaichi}) due to an impulse normal to the contact surface. Note that there is a small dent between the three circles, creating a local optimum.

% \textbf{Grasp} An environment that involves articulated objects based on nimble physics. Currently limited byw the platform, we designed the 3-DoF robot arm by hand. \citep{werling2021fast}.
% \textbf{Rope} We used Plasticine Lab \citep{huang2020plasticinelab}, which provides smooth gradients to evaluate on soft-body environment. Figure~\ref{}a shows four environments.

%\subsection{Evaluation of RPG on Rigid and Soft Body Manipulation Tasks}

%We first show that bayesian optimization.

%1. we replace the gradient-descent in our method to optimize the actor  2. We optimize the actor by directly descending its parameter on the reward landscape with Adam~\citep{adam} without including a latent distribution.

%We c 1. Sample efficiency and 2. converged trajectory and reward distribution, when the function class of reward involves local minima and discontinuities. 
%We evaluate our algorithms in several environments that . We analyze how these properties in reward landscape exert great challenge for single-modality action distribution and gradient-based methods.


We evaluate our method against the single modality policies learned from the following baselines: 1) Reinforce~\citep{williams1992simple}, and 2) policies optimized through path-wise gradients with Adam~\citep{adam}. We compare their sample efficiency and final performance after training is finished. 

\subsubsection{Experiment results} 
We plot the average episode return of each algorithm against the number of samples in Figure~\ref{fig:train_curve}.  
Error bars show the standard deviations over five runs with different random seeds.  The results suggest that our methods achieve better sample efficiency and find better solutions than baseline algorithms. 

% \textbf{Push} Push balls to avoid obstacles. We implement it by an impulse-based physical system similar to~[CITE: difftaichi]; 

% 3 several sampling-based methods, like training a population with reinitialization, CEM-MAS, and Bayesian optimization. 4. We evaluate popular deep reinforcement learning methods as a reference. Notice that our methods shall be able to combine with those methods when gradients do not exist. 
\begin{figure}[h]
    \begin{subfigure}[h]{1\textwidth}
    \centering
    % \includegraphics[width=1\textwidth]{figure/env_thumbnail.png}
    \includegraphics[width=0.8\textwidth]{figure/numerical_env_thumbnail.png}
    \caption{Environments for numerical experiments. We plot the reward landscapes in the first two bandit environments and show the rewards of the terminating positions as contour plots in the right three 2d move environments. These environments all pose some level of challenge in optimizing reward/value landscapes that are discontinuous and/or locally optimal.} \label{fig:envs}
    \label{fig:num_exps}
    \end{subfigure}
    
    \begin{subfigure}[h]{1\textwidth}
    \centering
    % \includegraphics[width=1\textwidth]{figure/sample_efficiency.png}
    % \includegraphics[width=1\textwidth]{figure/legends.png}
    \includegraphics[width=0.8\textwidth]{figure/numerical_exp.png}
    \includegraphics[width=0.8\textwidth]{figure/numerical_exp_legends.png}
    \caption{Training curve. X-axis: number of sampled states. Y-axis: average return. Error bars show standard deviations over 5 runs. Hyperparameters are available in Table \ref{tab:hyperparams}.} \label{fig:train_curve}
    \end{subfigure}
\end{figure}

% \textbf{Optimality}. 
% We can see that our method leverages the gradients, except when the gradient of reward is zero (Move 1).

We first take \textbf{Bandit 2} in Figure~\ref{fig:envs}-(2), which has two modes and regions containing zero gradients in its reward landscape, as an example for comparison. We show the performance of each algorithm in Figure~\ref{fig:train_curve}-(2).
In terms of optimality, our method converges to the globally optimal solution in the end and achieves a much higher return compared with other methods in Figure~\ref{fig:train_curve}-(2). %because of several advantages
%Thanks to our $\RELBO$ objective, the agent tends to explore 
Two reasons prevent our method from being stuck at the local optima. First, the entropy term in the $\RELBO$ objective encourages the agent to perform a maximum entropy exploration over the whole reward landscape, while the cross entropy term drives the agent to sample distinguishable actions for different latent variables, causing different action modes determined by latent variables to move away from each other, resulting in a better state coverage. 
Second, after discovering different local optima, our policy is able to maintain a multi-modality action distribution to exploit those local optima independently. By adjusting the probabilities of different modes through optimizing rewards with latent variables, it can eventually converge to the global optimal solution.
In experiments, we observed that although our method quickly found the right mode of the reward function, shown in Figure~\ref{fig:envs}-(2), which is locally optimal, it would still increase the probabilities for the under-explored region due to the exploration terms in our objective. After it found the left mode, it would maintain two action modes and optimize them together until the expected return of the left mode was larger than the right one and eventually converged to the left, finding the global optimum.

A notable feature of the multi-modality is that during the whole optimization process, the expected reward increases monotonically as it only needs to increase the reward for modes with higher rewards.
In contrast, when Adam and Reinforce converge to the right mode, even if we have introduced the maximum entropy reward to encourage exploration. different from our method, their single modality  property prevents them from jumping from one mode to a better mode as there is no way to go across the flat region in between without decreasing the reward.


In terms of sample efficiency, our method benefits from the pathwise analytical gradient, consistently outperforming Reinforce, which has a noisy gradient estimate that may reduce convergence speed when the number of samples is limited. Though Adam increases rewards faster than our method in the beginning stage, it quickly gets stuck at the local optima. Current RL algorithms like PPO or SAC are also constrained by the single modality gaussian parameterization of the policy, these methods can only find suboptimal solutions, even when more than enough samples are given.


\textbf{Remaining environments} 
Experiments on the remaining four environments show a similar behavior pattern that our method can converge to the global optima that the baselines fail to find.
We observe that the curve of ADAM in Figure~\ref{fig:train_curve}-(1) even decreases after reaching a local optimum. This is due to the discontinuity on the right of the reward landscape as shown in Figure~\ref{fig:envs}-(1). When a Gaussian policy reaches the right local optimum, the analytical gradients nearing that point still only contain a positive value, pushing the policy to go across the optimal point and move into the right flat region, causing the return to decrease to $-0.5$ in the end. Reinforce and PPO does not suffer from this issue, as it only uses the reward-weighted gradient estimate, and can correctly identify the left low-reward region and move away from it. SAC also does not suffer from this issue, as the policy optimizes the Q function, which smooth the discontinuity to allow the policy to converge at the local maximum stably. But it is still very challenging to find the global optima with a similar reason as in the \textbf{Bandit 2} environment. 

In the case of sequential decision-making problems, our method consistently outperforms algorithms that maintain single modality policy in several \textbf{move} environments by a large margin and can find global optima as shown in Figure~\ref{fig:train_curve} (3)-(5). We observed that Reinforce went to the left side mode in \textbf{Move 1} and \textbf{Move 2} as at the starting state there are no reward signals pointing to the global optimum in the upper side of the state space. Its variance is also high due to the increased problem dimensions. Adam even did not make any progress in \textbf{Move 1} as there is no gradient around the initial state. The \textbf{Move 3} environment includes physics-based contacts in the dynamic system, while our method still can solve it with the analytical gradients, in presence of the discontinuities during contacts. 

%REINFORCE shows a higher variance with increasing problem dimensions. Adam even doe
%The $2D$ move environments, similar to the bandit cases, 
%Single modality policy are unable to explore the multi-modalities  
% \begin{itemize}
%     \item In there Sample efficiency: Our method is always more sample efficient than REINFORCE. REINFORCE improves slower in the first 1M samples due to its log-likelihood ratio policy gradient estimator, which makes the update noisier and less efficient.%Our method converges to local optimum slower than Adam.: 
%     %\begin{itemize}
%     %\item Compare to Adam, our method optimizes ELBO that involves the entropy of latent variable, the entropy of action distribution, and a jointly optimized mutual information network, which can slow down the speed of optimization.
%     \item 
% \end{itemize}



% Figure 3a shows that our method and Adam, achieves faster policy improvement in the first 1M samples. Adam also improves slightly faster than our method since the reward composition is simpler than ours, which optimizes not only reward, but also entropy of both latent variable and action and their mutual information. REINFORCE is less sample efficient due to its log-likelihood ratio gradient estimator, which makes the update more noisy and less efficient. 

% Our method achieves the best final performance because its ability to maintain a more complex action/trajectory distribution. In this case，the first 1M samples, similar to REINFORCE and Adam, our method initially concentrated the action probability density on the right. Mutual information term in reward and the expressiveness of a reparameterized policy allow the action density conditioned on latent variable to shift across the flat reward region, and discovered the mode which contains global optimal reward. Then the latent shifts its sampling probability to the left mode of the reparameterized action distribution to optimize reward. Constrained by the expressiveness of action distribution, Adam and REINFORCE both suffered from the multi-modality landscape of reward.

% The remaining environments show similar behavior, our method outperforms baselines. In Bandit 2 as shown in Figure~\ref{}, we observe a drop of the ADAM. This is because .... In Move 1, explain the flat in the beginning. Move2; Move3.. Adam is good.  
% [In all environments] REINFORCE has a large variance than balbla. Although it can jump out of local optima because of its randness in  [Env, Env], it still can not find the global optima.

% These experiments show that 1.... 2...

% \textbf{Sample efficiency.} We observe that overall our method, like first-order gradient-based algorithms, such as Adam~\citep{adam} and our method, outperform REINFORCE at the initial stages (first 1e6 samples Bandit 1,2; Move 2,3). Initially, also because of optimizing on a simpler reward function than ours that does not optimize latent variable and its mutual information with actions, Adam converges into a local optimum much faster (first 1e6 samples Bandit 1,2; Move 2,3). However, discontinuity can completely stall the performance of Adam (Bandit 2, after around 1e6 samples), since the gradient direction does not always point to higher reward region, as shown in the reward function of Bandit 2. Our method which combines sampling and gradient also helps when the reward landscape is hard for a first-order method like Adam to optimize in all environments. First-order gradient-based methods obtain policy gradient from the gradient of reward/value directly, while REINFORCE estimates this gradient with a zeroth-order log-likelihood ratio estimator, which has higher variance. To achieve the same level of policy improvement as a gradient-based algorithm it will require more samples to estimate its gradient.

% \textbf{Final performance.} We observe in all 5 environments, our method achieves the best final performance. The performance of Adam suffers on flat (the states around center of Move 1) or discontinuous reward landscapes (right mode in reward of Bandit 2) due to its first-order gradient estimation, since the gradient direction does not always point to higher reward region, as shown in the reward function of Bandit 2 and Move 1. Although REINFORCE can escape discontinuities thanks to its reward-weighted gradient estimation, a single-modality Gaussian policy, which is of the same experiment setting as Adam, makes an algorithm hard to maintain a distribution of trajectory over the multi-modality of the reward landscape (right mode of reward for bandit environments, the 3 modes other than top mode for Move 1 and 2, and the small slot created by the obstacle). When there are multiple modes in reward, the action probability density of single-modality policy converges into the one that is closest to its initialization, which means, when the local optimum is closer to the initialization, it can easily get distracted by it and receive no further incentive to escape (all 5 environments). Besides, REINFORCE shows a high variance in performance across different seeds due to it's higher variance gradient estimator. It can easily get distracted by the outlier samples. To some extend, this also helps REINFORCE escape sparse reward region (the states around center of Move 1).
% On the other hand, our method combines the advantage of both sampling and gradient-based methods with the help of latent distributions. It enjoys the fast convergence of the gradient-based optimizer (first 1e6 samples of all 5 environments). Meanwhile, it can simultaneously search and explore the whole reward landscape under the maximum-entropy principle and finally find the optimal solutions (final performance of our method in all 5 environments). 



%The probability density of action quickly moves into a local maximum while not similar to the action conditioned on other latent variables by optimizing the elbo loss.

% {\small
% \begin{table}[H]
% \caption{Optimality: maximum/mean reward and the standard deviation over 5 runs; showing that we can better handle local optimum; RPG (reward-weighted gradient only) uses REINFORCE to update the reparamerized policy instead of using environment gradient. RPG (pathwise gradient only) very large $ent_z$, not able to select high-level $z$. %SAC/PPO for $z_dim=1$
% }
% \begin{center}
% \begin{tabular}{l||l|l|l|l}
% \toprule
% Algo$\backslash$Env & Bandit1 & Bandit 2& Move2D (Center Grad) & Move Local Max\\
% \midrule
% % RPG (Zeroth-order only)        & & & \\
% % RPG (First-order only)            & & & \\
% % \hline
% REINFORCE              & $-0.09 \pm 0.05$ & $-0.35 \pm 0.20 $ & $4.11 \pm 0.41$ &  \\
% ADAM                   & $-0.07 \pm 0.04$ & $-0.40 \pm 0.20 $ & $3.96 \pm 0.00$ & \\
% % \hline
% % SAC                    & & & \\
% % PPO                    & & & $0.04 \pm 0.07$ & \\
% RPG (ours)             & $\textbf{0.52} \pm 0.04$ & $\textbf{0.52} \pm 0.04$ & $\textbf{9.79} \pm 0.00$ & \\
% % \hline
% % Diffusion (REINFORCE) & & & \\
% % Diffusion (GD) & & & \\
% % Normalizing Flow (REINFORCE)  & & & \\
% % \hline
% % Reinitialization  & & & \\
% % CEM-AMS                & & & \\
% % Bayesian Optimization  & & & \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}
% }

%Here we demonstrate several properties of the reparameterized policy and explore several design choices.

%1. Effects of overparameterization for the optimization (number of hidden). more sample, more convex. \hza{effects of a number of $z_dim$}

%2. compare continuously and discretized hidden variables in a discontinuous environment,  \hza{roughly ok..}

% 3. showing the potential of exploiting discontinuity. 

%\hza{necessary}
%create a discontinuous environment, showing that GD can't stay at the global optima, but goes to other local optima.

%But our methods can keep the global distribution.

%4. Sequential hidden variable v.s. non-sequential variable.
%\hza{done. @ hza}

\subsubsection{How latent distributions affect the trajectory modeling?} 
Modeling the trajectories with a sequential $\{z_i\}$ instead of a single latent variable sampled before sampling the trajectory $\tau$ can help factorize the trajectory space to build a more compact representation. 
We construct an environment containing four obstacles to demonstrate its effects in Figure~\ref{fig:seqz}. The agent on the bottom left must avoid obstacles and reach the goal at the top right corner. We study the case where $z$ is a discrete variable.
We first plot the state and the action distributions for policies learned by sampling a single categorical $z$ before the trajectory $\tau$ in Figure~\ref{fig:sample before}.  Different colors represent the different values of $z$.
We plot the state and action distributions and use different colors to represent their corresponding $z$ values. Though a categorical distribution can represent various paths toward the goal, the number of latent samples constrained its expressive power. However, as shown in Figure~\ref{fig:sample after}, we model the distribution with a sequence of $z_1, z_{K+1}, z_{2K+1},\dots, z_{NK+1}$. This brings the compositionality that allows the agents to select various $z$ sequences to generate trajectories that can better cover the state space. The action distribution on the right successfully captures the symmetry of the optimal trajectories and the action pattern of moving along different directions, which helps the policy better cover the whole state space compared with a single categorical distribution.

% Nov 15

% but the choice of the latent space $\mathcal{Z}$ and the prior distribution $p(\mathcal{z})$  have a critical effect on the learned distributions.  
% When we only sample $z$ in begi
% %The first row shows the action distributions, colored by the value of $z$. 
% %In the first column of Figure~\ref{fig:seqz}(a), $z$ is sampled from a Gaussian distribution $\mathcal{N}(0, 1)$. 
% %The random noises are translated into various trajectories covering the whole state, while the actions tend to concentrate in the middle. When $z$ is formulated as categorical distribution

\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/sample_before.png}
         \caption{Sample $z$ before $\tau$}
         \label{fig:sample before}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/sample_after.png}
         \caption{Sample a sequence of $\{z_i\}$}
         \label{fig:sample after}
     \end{subfigure}
    \caption{A navigation task to demonstrate the effects of learning a sequence of $z$. An agent needs to move from the bottom left to the top right and avoid the green obstacles. Both the state and action space are $2$D. Different colors represent different values of $z$ or $z_i$.}
    \label{fig:seqz}
\end{figure}

\subsection{Evaluation on Manipulation Tasks with Differentiable Physics}
We evaluate our approach in several physical environments to demonstrate its potential in trajectory optimization. Figure~\ref{fig:diffphys_exp} compares our approaches against the gradient-based trajectory optimizer with a single Gaussian head in three environments. The \textbf{Grasp} environment, based on Nimble Physics~\citep{werling2021fast}, contains three balls. The agent needs to control a 3 DoF gripper to grasp the green ball and pick it up. However, the agent only knows that it needs to grasp an object, and it does not receive any reward before lifting it. We use a reward to minimize the distance between the gripper and the nearest balls, which creates a \textit{local minimum} that encourages the gripper to touch the nearest ball in front of it, as shown in Figure~\ref{fig:diffphys_exp}. The first-order gradient-based trajectory optimization got stuck. In contrast, our method can capture the multimodality of the reward landscape, approach different balls, and exploit different options (touching different balls) simultaneously. In the end, our method successfully finds the solution to pick up the green ball. The \textbf{Rope} and the \textbf{Cut} environments are two soft body environments built with PlasticineLab~\citep{huang2020plasticinelab}, each containing a 3DoF rigid body manipulator. In the \textbf{Rope} environment, an agent needs to push the left side of a rope forward.
Similarly, in the \textbf{Cut} environment, an agent needs to cut off the left end of a rope. However, manipulators are initialized in the middle of the objects, which is far away from suitable contact points required to finish the tasks, leading to local optima~\citep{li2021contact} as shown in Fig.~\ref{fig:diffphys_exp}. In contrast, our method can explore different contact points and find correct solutions in the end. These experiments show the potential of our approach in learning the optimal policies with differentiable physics.

%Our method also
% \hza{Limitation of the rigid body environments.} We notice a similar effects rigid body environments, the gradient 

% [we will plot the results of 4 environments. Nimble Grasp, Cut,Rope, Pus]

% Differentiable Physics Env ..
% add initial state or turn states into fade..
% Instability; remain for the future work.

% \begin{figure}[H]
%     \centering
%     % \includegraphics{}
%     \caption{Trajectory coverage curve. X-axis: simulator steps. Y-axis: discretized trajectory entropy. Color: algorithm.}
%     \label{fig:my_label}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/diff_phys.png}
    \caption{Visualization of policy distribution for manipulation with differentiable physics. We qualitatively compare the Gaussian policy learned by ADAM and the multi-modality policy learned by our method. On the left, we overlay final states from three trajectories of the Gaussian policy. On the right, we also draw three samples (trajectories) from the policy, and we visualize the final state of each trajectory in a different plot. We see that the three final states from the Gaussian policy are similar, while the final states are very different for trajectories from our policy. Additionally, one of the modalities of our method can solve the problem (the rightmost column), while the Gaussian policies get stuck in local minima.}
    \label{fig:diffphys_exp}
\end{figure}

% \begin{table}[H]
% \caption{Trained policy discretized trajectory distribution entropy and standard deviation over 5 runs.}
% \begin{center}
% \begin{tabular}{l|l|l|l|l|l}
% \toprule
% Algo$\backslash$Env  & Rigid2D Push  & Rigid3D Grasp & Rigid3D Locomotion & Soft3D Rope & Soft3D write \\
% \midrule
% PG (RL)              & & & & \\
% PG (GD)              & & & & \\
% RPG                  & & & & \\
% SAC                  & & & & \\
% PPO                  & & & & \\
% Population Learning  & & & & \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

% \textbf{Escaping Local-Optima}. To understand the difference in the capability of escaping local optimal solutions between algorithms, we modify the above environments slightly to form an obvious local minima in the solution space and repeat the above 2 evaluations: sample efficiency and multi-modality of solution.




==> text/infinite_horizon.tex <==
\section{Proof for Reparameterized Policy Gradient Theorem}
\label{appendix:rpg_proof}

In this section, we set up the condition for the existence of our reparameterized policy gradient. We focus on the continuous domain, where we can try to define gradients of the environment itself. We adopt a time-dependent reward formulation as we want to analyze both the finite horizon trajectory optimization and the infinite horizon Markov decision process together.
The existence of value function and value gradients in continuous space is obvious and might be considered folklore. However, the proof is often omitted in the traditional policy gradient course\footnote{For example, missing from the classical reinforcement learning textbook~\cite{sutton2018reinforcement}. The way to prove that a value function is differentiable from contraction mapping is not always obvious.}. Here we provide a simple analysis for rigorous\footnote{\todo{}check https://rltheory.github.io/lecture-notes/planning-in-mdps/lec16/}.

\subsection{Preliminaries}
\input{figure/graphical_model}

\subsubsection{Background and notations}
\todo{Notion and definition table.}

\paragraph{Trajectory Optimization} For simplicity, we consider a discrete dynamical system $f: \mathcal{S}\times \mathcal{A}\rightarrow \mathcal{S}$ defined on state space $\mathcal{S}$ and action space $\mathcal{A}$. The transition function $f$ transfers a state $s$ to a new state $s'=f(s, a)$ given an input action $a$.  Let state $s_1$ be the first time step, then we can iteratively apply the transition function by executing an action sequence $\mathbf{a}_T=\left\{a_1, a_2, \dots, a_T\right\}$ of length $T$. The system will produce state sequence $s_2,\dots s_{T+1}$ such that $s_{t+1}=f(s_t, a_t)$ for any $t$.

We use the term \textit{trajectory} to refer a sequence that contains both states and actions, e.g., $\tau_T=\{s_1, a_1, s_2, \dots, a_T, s_{T+1}\}$. Let's first assume $T$is finite, and $f$ is deterministic, then the trajectory becomes fully determined given the initial state and the action sequence, i.e., $\tau_T(s_1, \mathbf{a}_T)$.  In trajectory optimization problems, a reward function $R(\tau_T)$ maps the trajectory into a real value, representing how well the trajectory is w.r.t. the specified goal. We seek an action sequence $\mathbf{a}_T$ to maximize the trajectory reward $R(\tau_T)$. 

\paragraph{Reinforcement learning} or optimal control does not optimize an action sequence. Instead, it optimizes a parameterized policy $\pi_\theta(a|s):\mathcal{S}\times \mathcal{A}\rightarrow \mathbb{R}$, where $\theta$ is the policy parameter.  
Without loss of generality, let parameter $\theta\in \mathbb{R}$ \footnote{we can compute the gradients of multiple parameters individually.}.
The policy selects an action $a$ based on the current state $s$. For any $T$ and an initial state $s_1$, executing the policy will sample a trajectory of length $T$ where $a_t\sim \pi(a|s_t)$ and $s_{t+1}=f(s_t, a_t)$.
With the help of the policy, we can easily sample an infinite trajectory by letting $T\rightarrow \infty$. For convenience, we write a sampled infinite horizon trajectory  as $\tau=\{s_t,a_t\}_{t\ge 1}\sim \pi$ and $\tau_T=\{s_1, a_1, s_2, \dots, a_T, s_{T+1}\}$ as its finite prefix. Infinite horizon trajectories are very common in reinforcement learning as RL agents explore as many steps as possible in the environment until reaching the stationary distribution (mixing). 

Note that for any fixed $T$, the policy defines a distribution over all trajectories. Since we have seen that the trajectory is determined by the action sequence, $\tau_T=\tau(s_1, \mathbf{a}_T)$, we can see that the probabilistic density of a trajectory $\tau_T=\{s_1, a_1, s_2, a_2, \dots, a_T, s_{T+1}\}$ can be written as $$\pi(\tau_T)=p(s_1)\Pi_{t=1}^T\pi(a_t|s_t).$$

Policy optimization aims to find parameters to maximize expected future rewards. In another word, given the initial state $s_1$ sampled from a initial distribution $p(s_1)$, we want to maximize the \textit{value} $V^{\pi_\theta}$ of the policy $\pi_\theta$. Informally, we define the finite horizon value function, 
$$V_T^{\pi_\theta}(s)=E_{s_1=s, \tau_T\sim \pi_\theta}[R(\tau_T)]=E_{\tau_T\sim \pi_\theta(\cdot |s_1)}[\pi(\tau_T|s_1)R(\tau_T)],$$
and for the infinite case we have $$V^{\pi_\theta}(s)=\lim_{T\rightarrow \infty} V^{\pi_\theta}_T(s).$$
Note that value becomes a function of both parameter $\theta$ and the initial state $s_1$. The goal of policy optimization is to find parameters that maximize the value function, i.e., $$\theta^* = \arg\max_{\theta} E_{s\sim p(s_1)}[V^{\pi_\theta}(s)].$$
The trajectory reward $R(\tau)$ is usually defined as the sum of rewards per-step $\sum_{t\ge 1} R_t(s_t, a_t)$ in reinforcement learning so that it obeys the Markovian property. To guarantee the convergence of the sum of infinite per-step reward $\sum_{t=1}^\infty R_t$ so that the value function could be defined, it is enough to consider an exponential discounting reward $R_t=\gamma^t R$ which decays exponentially and has a bounded prefix sum. In this case, we can choose a large enough $T$ to approximate the total reward of an infinite horizon trajectory. We will show later that the value function exists under this special discounting scheme. On the other hand, a finite horizon trajectory could be alternatively viewed as the case that $R_t=0, \forall t>T$, which is another way to ensure that the value function could be well defined. 

Policy gradient methods~\cite{} solve the policy optimization problem by computing the gradients of the value function w.r.t. the policy parameters, i.e.,$\frac{\partial }{\partial \theta}V^{\pi_\theta}$ and gradient-based optimization methods to adjust the policy. 

\paragraph{Reparameterized Policy} 
The reparameterized policy uses a hidden random variable $z_t\in \mathcal{Z}$ to absorb randomness and model the action distribution $a_t=\pi_\theta(s_t, z_t)$ while $z_t\sim \pi_\theta(z_t|s_t, z_{t-1})$. The probabilistic graphical model is shown in Figure~\ref{fig:rpg}. We assume that $z_0$ is provided.

Similar to the action sequence, when we execute the policy $\pi_\theta(z_t|s_t, z_{t-1}), a_t=\pi_\theta(s_t, z_t)$, the policy will generate an action sequence $\mathbf{a}_T$ together with a $\mathbf{z}_T$ sequence. For convenience, we use the subscripts and bold letter $\mathbf{z}_{l:r}$ to represent a sequence $\{z_l,\dots, z_r\}$, $\mathbf{z}_T$ to represent $z_{1:T}$ and $\mathbf{z}$ to represent $z_{1:\infty}$. We still define $\tau_{l:r}=\{s_l, a_l, \dots, s_r, a_r\}$.
For any $t$, $\mathbf{a}, \mathbf{s}, \tau$ become functions of $\theta, s_1$ and $\mathbf{z}$.
For any $\mathbf{z}_T$, we can compute the corresponding probability $\pi_{\theta}(\mathbf{z}_T|s_1)=\prod_{i=1}^{T}\pi_\theta(z_t|s_t,z_{t-1})$ where $s_{t+1}=f(s_t, \pi_\theta(s_t, z_t))$. 

\todo{Special cases:}
\begin{itemize}
    \item The policy (without parameterization).
    \item Stochastic environments that could be reparameterized.
    \item Environments with various initial states.
    \item Note that here we assume that $z$ is a continuous variable. All conclusion holds that $z$ is categorical or mixing categorical, continuous variables. One can assume that we do integration over Dirac's delta function for discrete variables. 
\end{itemize}


\paragraph{Reparameterized Policy Gradient}
\todo{State that the trajectory becomes a function of z, and the probability of z is a determined function of $s_1$.}

We aim to compute the gradient of the following integral for $T\rightarrow \infty$.
$$\lim_{T\rightarrow \infty}\frac{\partial}{\partial\theta}V_T^{\pi_\theta}=\lim_{T\rightarrow \infty}\frac{\partial}{\partial \theta}\int_{\mathcal{Z}_T} \pi_\theta(\mathbf{z}_T)R(\tau_\theta(\mathbf{z}_T))d\mathbf{z}_T,$$ 
where $\mathcal{Z}_T$ denotes for the all possible $\mathbf{z}_T$ sequences, $V_T^{\pi_\theta}$ denotes for the value (expected reward) for length $T$ trajectories and $\frac{\partial}{\partial \theta}V_T^{\pi_\theta}$ is the policy gradient.
\todo{State the key theorems there.}


\subsubsection{Lemma}
To switch the order of integration/infinite sum:
\begin{lemma}[Fubini's theorem]
Suppose $X$ and $Y$ are $\sigma$-finite measure spaces and suppose that $X\times Y$ is given the product measure (which is unique as $X$ and $Y$ are $\sigma$-finite). Fubini's theorem states that if $f$ is $X\times Y$ integrable, meaning that $f$ is a measurable function and
$$\int_{X\times Y} | f(x, y) | d(x, y) < \infty$$
then 
$$\int_X\left(\int_Y f(x, y)dy\right)dx=\int_Y\left(\int_X f(x, y)dx\right)dy=\int_{X\times Y} f(x, y) d(x, y)$$
\label{lemma:fubini}
\end{lemma}

The continuity needs to be guaranteed by \href{https://math.stackexchange.com/questions/143124/continuity-of-parametric-integral}{Dominated convergence theorem}. See \href{https://encyclopediaofmath.org/wiki/Parameter-dependent_integral}{Parameter-dependent integral} and proof \href{https://www.uni-ulm.de/fileadmin/website_uni_ulm/mawi.inst.020/sauter/ws14/measure-theory.part3.2015-02-05.pdf}{this one..}

To differentiate under integration, we use the following \href{https://planetmath.org/differentiationundertheintegralsign}{condition},
\begin{lemma}[Leibniz integral rule, measure theory version] Let $X$ be an open subset of $\mathbb{R}$, and $\Omega$ be a measure space. Suppose that a function $f: X\times \Omega\rightarrow \mathbb{R}$ satisfies the following conditions:
\begin{enumerate}
    \item $f(x, \omega)$ is a Lebesgue-integrable function of $\omega$ for each $x\in X$.
    \item For almost all $\omega \in \Omega$, the derivative $\partial f(x, \omega)/\partial x$ exists for all $x\in X$.
    \item There is an integrable function $\Theta\rightarrow \mathbb{R}$ such that $|\partial f(x, \omega)/\partial x|\le \Theta(\omega)$ for all $x\in X$.
\end{enumerate}
\label{lemma:leibniz}
Then for all $x\in X$, $$\frac{d}{dx}\int_{\Omega}f(x, \omega)d\omega=\int_\Omega\frac{\partial }{\partial x}f(x, \omega)d\omega$$
\end{lemma}

To ensure the continuity of the value function and the value gradient, we use the \href{https://people.math.wisc.edu/~angenent/521.2017s/UniformConvergence.html}{uniform convergence} condition in the following theorems.

\begin{lemma}
Let $f_n:E\rightarrow \mathbb{R}$ be a sequence of functions. If $f_n$ converges uniformly to $f:E\rightarrow \mathbb{R}$, and if each $f_n$ is continuous, then f is also continuous. 
\label{lemma:continuousoflimit}
\end{lemma}
%\begin{theorem}[switch limits and integration]
%If $f_n:[a,b]\rightarrow R$ is a sequence of Riemann integrable functions that converges uniformly to $f:[a,b]\rightarrow R$, then the limit $f$ is also Riemann integrable and 
%$$\lim_{n\rightarrow \infty}\int_a^b f_n(x)dx=\int_a^b f(x) dx.$$
%\label{theorem:switch_limit_integration}
%\end{theorem}

Then by \href{https://web.math.ucsb.edu/~agboola/teaching/2021/winter/122A/rudin.pdf}{Theorem 7.17 in Rudin's analysis, p152} we have\footnote{we do not need the continuity of the derivative, but by the remark, if we have it, the proof could be much simpler.}
\begin{lemma}[switch limits and derivative]
Let $f_n:[a,b]\rightarrow \mathbb{R}$ be a sequence of differentaible functions.
If $f_n$ converges uniformly to $f$ and $f'_n$ converges uniformly to $g$, then the limit $f$ is differentiable and its derivative is $f'=g$, i.e.,
$$\lim_{n\rightarrow \infty}\frac{df_n(x)}{dx}=\frac{d\lim_{n\rightarrow \infty}f_n(x)}{dx}.$$
\label{lemma:switch_limit_deriative}
\end{lemma}




%For any $\mathbf{z}$ that $p_{\theta}(\mathbf{z})>0$, 
\subsection{Regularity conditions}
We assume the following regularity conditions for all remaining parts.
%\begin{assumption}[Compactness and complete]
%the state space $\mathcal{S}$, the parameter space $\theta\in X$, and the action space $\mathcal{A}$ are compact (and complete), so that we can bound every continuous functions.  \label{assumption:compact}
%\end{assumption}
%Note that this is a very strong condition assumed in \cite{silver2014deterministic}, while in \cite{suh2022differentiable} admits a much lossen condition. The compactness should be quite easy to achieve in practice. \hza{I guess All of the requirements here could be replaced by finite moments/Lebesgue integrable or something else. Currently let's bound everything to simplify the prove. Besides, we do not need the hidden space $\mathcal{Z}$ to be compact, just need it to be integrable.}

\begin{assumption}
The policy $\pi_\theta(z'|s, z)$ satisfies
\begin{itemize}
    \item Lipschitz continuous w.r.t. $\theta$.
    \item Lebesgue integrable for all $z$ and dominated convergence.
    \item $\exists M, \forall T$, there is a Lebesgue integrable function $g$ such that $ \mathbf{z}_{T-1}, |\nabla_\theta \pi(z_T|\mathbf{z}_{T-1})|\le g(z_T|\mathbf{z}_{T-1})$ and $\int g(z_T|\mathbf{z}_{T-1}) dz_T\le M$ (dominated convergence).
\end{itemize}
\label{assumption:Lipschitz}
\end{assumption}
Lipschitz is guaranteed by neural networks. Categorical distribution or a finite mixture of gaussian should satisfy the dominated convergence condition. \hza{But we have not proved that for Gaussian's gradients.}

Note that this assumption rules out the deterministic policy, as functions involving the Dirac delta function are usually not Lipschitz.
\begin{assumption}[Lipschitz environment]
In addition to the policy, we require the dynamics and the reward $s'=f(s, a), R_t(s, a)$ to be Lipschitz continuous w.r.t. $s, a$. \label{assumption:Lipschitz_env}
\end{assumption}

\paragraph{Dominated convergence of Gaussian Mixture} Regarding the Lipschitz condition of the probability, we only need this to ensure the density's gradient is bounded. This holds for Gaussian policy with a fixed range (for any trajectory) $\sigma$ range (bound by $ce^{-a(x-b_{\text{min}})^2} + ce^{-a(x-b_{\text{max}})^2}$ for large enough $c$ and small enough $a$). As for the gradients, it is the gradients of $\int e^{-t} dt$ where $t=(x-\mu)$ after substitution. However, if we allow $\sigma\rightarrow 0$ in our policy execution and $\mathcal{Z}$ is not compact. both the derivative w.r.t. $\mu$ and $\sigma$ are not bounded. Just don't do this...

%/*\hza{Additional conditions about rewards.}
%\textbf{No exploding gradient condition} For $p(\mathbf{z})>0$, The absolute sum of gradient $\nabla_{s_i, a_i} R(\tau_\theta(\mathbf{z}))$ converges and is bounded for all $s_i, a_i$. This could happen for finite horizon, where the reward is a Lipschitz function on the compact set, or when the decay factor is large and can discard chaotic behaviors in a Lipschitz continuous system. \hza{Can we bound the gradients of the system even when there are additional gradients of $a_i$ w.r.t. $s_i$ through the policy network?} \hza{This is not the necessary condition as we only need the gradients to be Lebesgue integrable given the current policy.}*/

\subsection{The existence of value function}
We use the following assumption to ensure the existence of the value function $V^{\pi_\theta}=\lim_{T\rightarrow \infty}V_T^{\pi_\theta}$. 

%\begin{assumption}[Uniform convergence of reward sum]
%\end{assumption}

\begin{corollary}[Existence of finite horizon value]
If for any $\mathbf{z}, \theta$ the reward prefix sum sequences $R(\tau_\theta(\mathbf{z}_T))$ is bounded by $R_{\text{max}}$, and converges uniformly to $R(\tau_\theta(\mathbf{z}))$; if \textbf{$\pi_\theta(\mathbf{z}_T)R(\tau_\theta(\mathbf{z}_T))$ are continuous w.r.t. $\theta$ for any $T, \mathbf{z}_T$}, then the function sequence $\{V_T^{\pi_\theta}\}_{T\ge 1}$ about $\theta$ convergences uniformly and the limit $V_T^{\pi_\theta}$ exits. %and the limit is continuous w.r.t. $\theta$.
\label{corollary:value_continuous}
\end{corollary}
\begin{proof}
First we show that for any $T$, $V_T^{\pi_\theta}$ exists and continuous w.r.t. $\theta$. This is obvious as we have assumed that the trajectory contribution $\pi_\theta(\mathbf{z}_T)R(\tau_\theta(\mathbf{z}_T))$ are continuous function w.r.t. $\theta$ and bounded by Lebesgue integrable function $\pi_\theta(\mathbf{z}_T)R_{\text{max}}$ based on Assumption~\ref{assumption:Lipschitz}. The integration $\int_{\mathcal{Z}_T}\pi_\theta(\mathbf{z}_T)R(\tau_\theta(\mathbf{z}_T))d\mathbf{z}_T$ exists. If the probability satisfies the \todo{dominated convergence condition}, it becomes a continuous function of $\theta$.

To prove that the limitation $\lim_{T\rightarrow \infty}V_T^{\pi_\theta}$ exists. By the uniform convergence of $R(\tau_\theta(\mathbf{z}_T))$, for any $\epsilon, \exists T_\epsilon, \forall, \theta, \mathbf{z},  T_2>T_1>T_\epsilon \Rightarrow | R_{T_1}-R_{T_2}|<\epsilon \Rightarrow$
\begin{align*}
V_{T_2}&=\int \pi_\theta(\mathbf{z}_{T_2})\left(R_{T_1} + R_{T_2}-R_{T_1}\right) d{\mathbf{z}_{T_2}}\\
&=\int R_{T_1}\pi_\theta(\mathbf{z}_{T_1})\pi_\theta(\mathbf{z}_{T_1+1:T_2}|\mathbf{z}_{T_1})d{\mathbf{z}_{T_2}} + \int \pi_\theta(\mathbf{z}_2)(R_{T_2}-R_{T_1}) d{\mathbf{z}_{T_2}}\\
&=\int R(\mathbf{z}_{T_1})\pi_\theta(\mathbf{z}_{T_1})\left(\int \pi_\theta(\mathbf{z}_{T_1+1:T_2}|\mathbf{z}_{T_1}) d\mathbf{z}_{T_1+1:T_2}\right) d\mathbf{z}_{T_1} + O(\epsilon)\\
&=V_{T_1}+O(\epsilon),
\end{align*}
which is still a Cauchy sequence and thus converges uniformly for all $\theta, \mathbf{z}$.
The left part in the third step is guaranteed by the Lemma~\ref{lemma:fubini} that we can swap integration signs for absolutely integrable function. The right side part is guaranteed by the Lebesgue integrability of our $\pi_\theta$.

When each $V_{T}$ is continuous provided by the dominated convergence condition, by Lemma~\ref{lemma:continuousoflimit}, $V_T^{\pi_\theta}$ is a continuous function w.r.t. $\theta$.
\end{proof}

\subsection{The existence of the policy gradient} We first set up the condition for the existence of the original policy gradients in the continuous domain.  We include it here for a better understanding of the differentiable cases. 

We first use the following \href{https://math.stackexchange.com/questions/1028974/sum-and-product-of-lipschitz-functions}{lemma}
\begin{lemma}
For $n$ $L$-Lipschitz function $0 \le \pi^i(x)\le B$, their product is still $nLB^{n-1}$-Lipschitz and bounded by $B^n$. However, if their gradients are all absolutely integrable and the integration is bounded by $M$, then their products are also absolutely integrable and bounded by $nM$. \label{lemma:nLipschitz}
\end{lemma}
\begin{proof}
We can prove by induction. For two function $f, g$ of $L_1$ and $L_2$ Lipschitz, we have 
\begin{align*}|f(x)g(x) - f(y)g(y)|&\le |f(x)g(x)-f(x)g(y)|+|f(x)g(y)-f(y)g(y)|\\&\le |f(x)||g(x)-g(y)| +|g(y)||f(x) - f(y)|\le (L_1+L_2)|x-y|\max(f(x), g(y)).
\end{align*}
Then it is obvious.

The Lipschitz condition ensures that the gradients exist almost everywhere and are bounded. Since we further assume that for all $T+1$, each gradient is absolutely integrable and always bounded, which means that $\int |\nabla \pi(z_{T+1}|\mathbf{z}_{T})|dz_{T+1}<M$ and notice that $\pi\ge 0$, then by induction, $\forall T$,
\begin{align*}
\int_{\mathcal{Z}_T}|\nabla \pi(\mathbf{z}_T)|d\mathbf{z}_T
&=\int_{\mathcal{Z}_T}|\nabla \pi(\mathbf{z}_{T-1})\pi(z_T)|d\mathbf{z}_T\\
&=\int_{\mathcal{Z}_T}|\pi(z_T|\mathbf{z}_{T-1})\nabla \pi(\mathbf{z}_{T-1}) + \pi(\mathbf{z}_{T-1})\nabla\pi(z_T|\mathbf{z}_{T-1})) |d\mathbf{z}_T\\
&\le \int_{\mathcal{Z}_T}|\pi(z_T|\mathbf{z}_{T-1}))\nabla \pi(\mathbf{z}_{T-1})| + |\pi(\mathbf{z}_{T-1})\nabla\pi(z_T|\mathbf{z}_{T-1})) |d\mathbf{z}_T\\
&= \int_{\mathcal{Z}_{T-1}}\int_{z_T}\pi(z_T|\mathbf{z}_{T-1})dz_T\left|\nabla \pi(\mathbf{z}_{T-1})\right|d_{\mathbf{z}_{T-1}} + \int_{\mathcal{Z}_{T-1}}\pi(\mathbf{z}_{T-1})\int_{z_T}|\nabla\pi(z_T|\mathbf{z}_{T-1})) |d{z_T}d\mathbf{z}_{T-1}\\
&\le M(T-1) + M\le MT
\end{align*}
\end{proof}


\begin{corollary}
We assume that $a_t=\pi(s_t, z_t)$ is a deterministic function irrelevant to $\theta$ (for example $a_t$ is simply $z_t$) as shown in Figure~\ref{fig:pg}. Under the conditions in Corollary~\ref{corollary:value_continuous} and assume that reward sequence $R(\mathbf{z}_{T+1})-R(\mathbf{z}_{T})$ is $O(\frac{1}{T^3})$. The for any $T$, the value $V_T^{\pi_\theta}$ is differentiable, its gradient $\frac{\partial}{\partial \theta}  V_T^{\pi_\theta}$ converges, and the limitation is $\frac{\partial }{\partial \theta}V^{\pi_\theta}$.\label{corollary:policy_gradient_turn}
\end{corollary}
\begin{proof}
In this case $\tau(\mathbf{z}_t), R(\mathbf{z}_t)$ is purely a function of $\mathbf{z}_t$ but not $\theta$. Then,
$$V_T^{\pi_\theta}=\int \prod_{t=1}^T\pi_{\theta}(z_t|s_t,z_{t-1}) R(\mathbf{z}_T)d\mathbf{z}_T,$$
is the integration of function $\pi_{\theta}$ times the trajectory reward. Since $R$ is bounded (under assumption , $\pi_\theta$ is bounded, their product is bounded, and differentiable almost everywhere and Lipschitz w.r.t. $\theta$ (because Lemma~\ref{lemma:nLipschitz}). Note that when $\mathbf{z}$ is fixed, $R$ is not a function of $\theta$. We can apply the generalized Leibniz integral rule (Lemma~\ref{lemma:leibniz}) and the likelihood trick, in this case, the value is differentiable and 
\begin{align*}
    \frac{\partial}{\partial \theta}V_T^{\pi_\theta}&=
    \int \frac{\partial}{\partial \theta} \prod_{t=1}^T\pi_{\theta}(z_t|s_t,z_{t-1}) R(\mathbf{z}_T)d\mathbf{z}_T\\
    &=\int \prod_{t=1}^T\pi_{\theta}(z_t|s_t,z_{t-1}) \left(\sum_{i=1}^T\frac{\partial}{\partial \theta}\log \pi_\theta(z_t|s_t,z_{t-1})\right) R(\mathbf{z}_T)d\mathbf{z}_T \\
\end{align*}
To apply Lemma~\ref{lemma:switch_limit_deriative}, we need value $V_T^{\pi_\theta}$ and its gradient uniformly converges. The continuous of $V_T^{\pi_\theta}$ and uniformly converges\footnote{We do not assume the derivative is continuous.. actually it is not true for the neural networks.} is guaranteed in Corollary~\ref{corollary:value_continuous} because of the Lipschitz continuity of $\pi_\theta(\mathbf{z}_T)R(\mathbf{z}_T)$.
\footnote{\textbf{Notice that $\log \pi_\theta$ may be not  \href{http://www.math.jyu.fi/research/reports/rep100.pdf}{Lipschitz}.}} %, we can choose $T$ such that $\left|\frac{\partial}{\partial \theta} \log \pi_\theta(z_T|s_T, z_{T-1})r(s_T, z_T, a_T)\right|\le \epsilon$ and notice that $\int \log \pi_\theta(z_T|s_T, z_{T-1})R(\mathbf{z}_T)d z_T=0$ we can eliminate residual at time step $T$ to prove the convergence.
$R(\mathbf{z}_T)-R(\mathbf{z}_{T+1})$ is $O(\frac{1}{T^3})$ implies that for large enough $T$, $\exists C$ such that $|R_{T+1}-R_T|<\frac{C}{T^3}\Rightarrow$ for almost surely existing $\nabla \pi_\theta$, $\int_{\mathbf{Z}_{T+1}} \nabla \pi_\theta(\mathbf{z}_{T+1})|R_{T+1}-R_T|<\frac{MC}{T^2}$ is $O(\frac{1}{T^2})$ as $\nabla \pi_\theta(\mathbf{z}_{T+1})$ is Lipschitz continuous, so
\begin{align*}
\nabla V_{T+1}&=\int \nabla \pi_\theta(\mathbf{z}_{T+1})\left(R_{T+1} + R_{T+1}-R_{T}\right) d{\mathbf{z}_{T+1}}\\
&=\int \nabla \pi_\theta(\mathbf{z}_{T})\pi_\theta(z_{T+1}|\mathbf{z}_T)R_T d{\mathbf{z}_{T+1}} +O(\frac{1}{T^2})\\
&=\int \int \left(\pi_\theta(z_{T+1}|\mathbf{z}_T)\nabla \pi_\theta(\mathbf{z}_{T}) + \pi_\theta(\mathbf{z}_T)\nabla \pi_\theta(z_{T+1}|\mathbf{z}_T)\right)R_T dz_{T+1}d{\mathbf{z}_T} +O(\frac{1}{T^2})\\
&=\nabla V_T + 0 + O(\frac{1}{T^2}).
\end{align*}
The first term could be simplified as $\int \pi_\theta(z_{T+1}|\mathbf{z}_T)dz_{T+1}=1$. The second term is zero as $\int \nabla \pi_\theta(z_{T+1}|\mathbf{z}_T)dz_{T+1}=0$. The first part is simply $\frac{\partial}{\partial \theta}V_T$. 
Then by \href{https://en.wikipedia.org/wiki/Direct_comparison_test}{direct comparison test} we know that the $|\nabla V_{T+1}-\nabla V_T|$ is bounded by $O(1/T^2)$, which converges uniformly for all $\theta$. Thus we have $\lim_{T\rightarrow \infty}\frac{\partial }{\partial \theta} V_T^{\pi_\theta}=\frac{\partial }{\partial \theta}V^{\pi_\theta}$ by Lemma~\ref{lemma:switch_limit_deriative}.
\end{proof}

\subsection{The conditions for reparameterized policy gradient}
The differences between the first-order estimator and the zero-order estimator have subtle differences. Despite different sample complexities, two factors will affect the correctness. First, it is possible that although policy gradients exist, when we allow the gradients to back-propagate through actions and states, the gradients could be unbounded. This happens in a chaotic system. Second, even if we can compute the derivative correctly when we apply Leibniz integral rule to switch derivative and the integration to formulate a sampling-based estimator, the gradient will be biased as it does not consider the integration boundary. Though we can compute the bias under mild conditions by integration over the boundary around that discontinuous point, it would be extremely challenging for high-dimensional cases.
\hza{this is used to prove the optimal control's stability}

%We define $V^i_T(s_i, z_{i-1})=\int_{\mathbf{z}} p_\theta(z_{i:T})R(\tau_\theta(z_{i:T}))d\mathbf{z}_{i:T},$ whose limit $V^i(s_i, z_{i-1})=\lim_{T\rightarrow \infty}V^i_T(s_i, z_{i-1})$ exits with a similar reason for $i=0$.

%If for any possible $\mathbf{z}$, $\lim_{T\rightarrow\infty}\frac{\partial R_t(\tau_\theta(\mathbf{z}_t))}{\partial \theta}$ converges superlinearly and bounded.
%, derivative, $\partial V_T^i(s_i, z_{i-1})/\partial \theta$

\begin{corollary}
Under assumption~\ref{assumption:Lipschitz},\ref{assumption:Lipschitz_env} and additional assumptions that the reward function converges in $O(\frac{1}{L^{2n}})$, the per time step's reward's Lipschitz decay in $O(\frac{1}{L^{2n}})$\footnote{this could be easily guaranteed by a discount $\gamma L^2<1$}. In this case, the value and value gradient exits and could be computed by derivative under the integration.
\end{corollary}
\begin{proof}
Let $\mathcal{L}_T(\mathbf{z}, \mathbf{s})=\pi_\theta(\mathbf{z}_T)R(\tau_\theta(\mathbf{z}_T))$, for any $\theta, \mathbf{z}_T$. Here is our proof sketch.
\begin{itemize}
    \item prove that $\mathcal{L}_T(\mathbf{z}, \mathbf{s})$ is Lipschitz w.r.t. $\theta$. Thus it can guarantee the almost everywhere differentiable of $\nabla \mathcal{L}_T$ and bound it. % to enable the differentiability under the integration and apply the Fubini's theorem.
    \item Using the derivative of the product to divide the gradients into two parts and try to bound both terms. Since the dynamical system will enlarge the gradient by at most $L^n$, it is always bounded and integrable because of the dominated integrable.
    \item prove that $\lim_{T\rightarrow \infty}\nabla \mathcal{L}_T$ converges under certain requirements for the reward sequences. 
    \item Then, by Lemma~\ref{lemma:switch_limit_deriative}, we prove the existence of the value gradients.
\end{itemize}

Let's first bound $\mathcal{L}_T(\mathbf{z}, \mathbf{s})$. Let $L_\pi, L_R, L_f$ be the Lipschitz constant of $\pi_\theta$, $R_i(s_i, a_i)$, $f(s_i, \pi_\theta(s_i, z_i))$ for simplicity. After fixing $\mathbf{z}_T$, we can easily prove that $s_n$ becomes a $L_f^n$-Lipschitz function by compositionality by induction. Then $\pi_\theta(\mathbf{z_T})$ becomes a Lipschitz function of $\sum_{i=1}^T L_\pi L_f^n$ and $R(\tau_\theta(\mathbf{z}_T))$ is bounded. The resulting function must be Lipschitz, so $\mathcal{L}_T(\mathbf{z}, \mathbf{s})$ is differentiable almost everywhere and is bounded. In this case, we can do integration over $\mathcal{Z}_T$ and compute the integration by Lemma~\ref{lemma:leibniz}
$$\frac{\partial}{\partial \theta}\int_{\mathcal{Z}_T}\mathcal{L}_T(\mathbf{z}_T, \mathbf{s}_T)d\mathbf{z}_T=\int_{\mathcal{Z}_T}\frac{\partial}{\partial \theta}\mathcal{L}_T(\mathbf{z}_T, \mathbf{s}_T)d\mathbf{z}_T.$$

We now ensure the convergence of the previous integration. We first have 
$$\int \frac{\partial }{\partial \theta} \mathcal{L}_T d\mathbf{z}_T= \int R(\tau_\theta(\mathbf{z}_T))\frac{\partial}{\partial \theta} \prod_{i=1}^T \pi_\theta(z_i|z_{i-1}, s_i) +\prod_{i=1}^T \pi_\theta(z_i|z_{i-1}, s_i) \frac{\partial }{\partial \theta}R(\tau_\theta(\mathbf{z}_T)) d\mathbf{z}_T.$$

With a similar reason to Corollary~\ref{corollary:policy_gradient_turn}, since $R$ converges and we only need $\nabla \pi_\theta(\mathbf{z})\Delta R$'s prefix sum converges, then the first part of the integration converges uniformly\footnote{Need to reorganize the prove in Corollary~\ref{corollary:policy_gradient_turn} to make this more obvious.}.
To bound the second part, just notice that $R(\mathbf{z}_{T+1}) - R(\mathbf{z}_{T+1}) = R_{T+1}(s_{T+1}, a_{T+1})$, we only need to ensure that the prefix sum of $\partial R_{T+1}/\partial \theta$ converges, which is guaranteed by the fast convergence rate of the rewards.
\end{proof}
%is bounded by $R_{\text{max}}L+L^2$,
%and we can then collect the gradients by 
%$$\frac{\partial  }{\partial \theta} \mathcal{L}_T = \sum_{i=1}^T \frac{\partial s_i }{\partial \theta}\frac{\partial \mathcal{L}_T}{\partial s_i}.$$

%The Lipschitz continous tells us that $\frac{\partial s_i}{\partial \theta}$ is  $O(L^T)\Rightarrow \frac{\partial }{\partial \theta}$. 

%The contribution of the first part, will contribution to each state $s_i$ a gradient of at most $ML$ where $M$ is the bound of the reward and $L$ is the Lipschitz constant of $\pi_\theta$. However, if we find a large enough $t$, such that the $R(b)$ part is negligible, we shall be able to prove that the gradient of $\pi(b)$, w.r.t. the whole state trajectories, is negligible.
%$$\int_{a} \pi(a) \int_{b} \left[R(a) + R(b)\right]\pi(b) db da,$$

%Consider any finite trajectories. The convergence requires that the individual gradients of $R$ and $\pi$ contributes at most $\frac{1}{T^2L^T}$ to the state so that the gradients after back-propogation will be bounded. For $\pi_\theta$, its contribution will be the previous reward plus the reward later. The part before is just the bias and could be ignored in the policy gradients, and thus its contribution is just the sum of the remaining rewards. Under this condition, we can bound the total gradients of the states and thus the gradient of $\theta$. In this case, we should be able to prove that it is uniformly convergence.
%When the gradient is bounded, the convergence of the gradients is obvious as $V_T$ and $V_T'$ are continuous and uniformly convergence.
%\href{https://people.math.wisc.edu/~angenent/521.2017s/UniformConvergence.html}{uniformly convergence}

==> text/intro_hao.tex <==
\section{Introduction}

% Story:
% - the multimodal policy is necessary for the exploration
% - the latent variable model enables a simple way to parameterize
% - when combined with reward maximization; enable jumping out of the local optima
%     - Toy curve; bandit tasks (illustrate why it succeeds)
%     - Cabinet or AntEnvs, BlockPickup （rewards with local optima)
%     - baselines: TDMPC; Mixture of Gaussian Policy
% - when combined with RND for sparse reward task; enable accelerated exploration and solve tasks efficiently
%     - experiments: sparse reward tasks
%         - four rooms
%             1. RND does not converge
%             2. slow coverage
%     - baselines: naive exploration; sac;

% \begin{itemize}
%     \item We demonstrate the effectiveness of a multi-modal policy for exploration in continuous space (we need to show why exploration with rewards is better than unsupervised learning).
%     \item We evaluate and analyze different representation learning for policy and show their benefits: Environments: 1. motion planning; 2. locomotion; 3. standard environment (antmaze); 4. manipulation. Baselines: skill discovery and HRL.
%     \item A simple variational policy learning framework that unifies representation learning and reward maximization.
% \end{itemize}

Reinforcement learning (RL) with \emph{high-dimensional continuous action space} is notoriously hard despite its fundamental importance for many application problems such as robotic manipulation~\citep{openaiHand, mu2021maniskill}. Compared with the discrete action space counterpart setup, it is much trickier to represent policies for continuous RL -- by the optimality theory of RL, the function class of discrete RL policies is simply categorical distributions~\citep{sutton2018reinforcement}, while the function class of continuous RL policies has to include density functions of arbitrary probabilistic distributions. 
            
In practice, popular frameworks~\citep{silver2014deterministic, haarnoja2018soft, schulman2017proximal} of deep RL formulate the continuous policy as a neural network that outputs a single-modality density function over the action space (e.g., a Gaussian distribution over actions). This formulation, however, breaks the promise of RL being a global optimizer of the return function because the single-modality policy parameterization introduces local minima that are hard to escape using gradients w.r.t. distribution parameters. Besides, a single-modality policy will significantly weaken the exploration ability of RL algorithms because the sampled actions are usually concentrated around the modality. Our Bandit examples show how a single-modality RL policy fails to solve a simple continuous action bandit problem. Therefore, in practice, continuous RL often requires meticulous reward design that takes considerable human effort~\citep{mu2021maniskill, savva2019habitat, yu2020meta, makoviychuk2021isaac, zhu2020robosuite}.


In this paper, we propose a principled framework to learn the continuous RL policy as a multi-modality density function. We provide a holistic solution to two closely-related questions: \emph{1) how to parameterize the continuous RL policy?} \emph{2) how to update the  policy parameterized as in (1)?} 
            
Our parameterization of the continuous RL policy is based on two ideas. First, we take a sequence modeling perspective~\citep{chen2021decision} and view the policy as a density function over \textit{the entire trajectory space} (instead of the action space)~\citep{ziebart2010modeling, levine2018reinforcement}. Under this sequence modeling perspective, we can sample a population of trajectories that cover multiple modalities of trajectories, which allows us to concurrently explore distant regions in the solution space. Second, we use a generative model to parameterize the multi-modality policies, inspired by their success in modeling highly complicated distributions such as natural images~\citep{goodfellow2016deep, zhu2017unpaired, rombach2022high, ramesh2021zero}. We introduce a sequence of latent variables $z$, and we learn a decoder that ``reparameterizes'' the random distribution $z$ into the multi-modality trajectory distribution~\citep{kingma2013auto}, from which we can sample trajectories $\tau$. Our policy network is, in a spirit, akin to diffusion models~\citep{rombach2022high, ramesh2021zero} by learning to model the joint distribution $p(z, \tau)$. As a prototypical work, we prefer simple design and choose not to include the multi-step diffusion process as in image modeling.

Our choice of policy parameterization leads us to adopt the variational method~\citep{kingma2013auto, haarnoja2018soft, moon1996expectation} to derive an on-policy learning algorithm. Classical on-policy learning leverages the policy gradient theorem~\citep{sutton2018reinforcement}, i.e., $\nabla J(\pi)=\mathbb{E}_{\tau}[R(\tau)\nabla\log p(\tau)]$. Because we model $p(z, \tau)$, that requires computing $p(\tau)$ and its gradient with $\int_z p(z, \tau)\,\mbox{d}z$. However, marginalizing out $z$ is often intractable when $z$ is continuous, and it is well-known that optimizing the marginal distribution $\log\,p(\tau)$ by gradient descent suffers from local optimality issues (e.g., using gradient descent to optimize Gaussian mixture models which have latent variables is not effective, so EM is often used instead~\cite{ng2000cs229}). To overcome these obstacles, we take a different route and adopt variational method (maximum entropy RL) that directly optimizes the joint distribution of the optimal policy without hassels of integrating over $z$. 

We derive a novel variational bound which is the optimization objective for policy learning. To maximize this objective, we introduce the \textbf{Reparameterized Policy Gradient Theorem}.     The theorem states a principled way to compute the policy gradient by combining the reward-weighted gradient (as in the classical policy gradient theorem) and the path-wise gradient from a differentiable world model (as in classical trajectory optimization methods). The two sources of gradient complement each other -- the reward-weighted gradient improves the likelihood of selecting trajectories from regions containing high-reward ones, whereas the path-wise gradient suggests updates to make local improvements to trajectories. This combination allows us to enjoy the precise gradient computation from differentiable world models~\citep{werling2021fast,hu2019difftaichi, huang2021plasticinelab} and also maintains the flexibility to sample and optimize the trajectory distribution globally. Note that this beautiful result is also a consequence of introducing the latent variable $z$.

The effectiveness of our method is rooted in our choice of generative policy modeling method. An ideal method needs to be powerful in modeling multi-modality distribution, and it needs to support sampling, density value computation, and stable gradient computation. Although there are other candidates for deep generative models, they often have limitations to being used for continuous policy modeling. For example, GAN-like generative models~\citep{goodfellow2020generative} can only sample but not compute the density value. While normalizing flow~\citep{rezende2015variational} can compute the density value, they might not be as robust numerically due to the dependency on the determinant of the network Jacobian; moreover, normalizing flows must apply continuous transformations onto a continuously connected distribution, making it difficult to model disconnected modes~\citep{rasul2021autoregressive}.


%[introduce experiment results]
We apply our methods to several numerical problems and three trajectory optimization tasks to manipulate rigid-body objects and deformable objects supported by differentiable physics engines~\citep{werling2021fast, huang2020plasticinelab}. These environments contain various local optima that challenge single-modality policies (either reward-weighted policy gradients as in REINFORCE or path-wise gradients as in trajectory optimization). In contrast, our approach benefits from modeling the trajectories as generative models and the ability to sample in the trajectory space. In qualitative experiments, we observe a strong pattern of multi-modality distribution by visualizing the policy after the learning converges. By quantitative evaluation, the policy learned by our framework does not suffer from the local optimality issue and significantly outperforms baselines.

==> text/intro_legacy.tex <==
\section{Introduction}

Broadly speaking, two primary methods for learning policies in (continuous) decision-making are sampling-based and gradient-based. [FIGURE HERE] Sampling-based methods like REINFORCE and evolutionary algorithms maintain policy distributions and optimize those distributions by trial and error. Such methods do not assume the underlying structures of environments and can usually explore the whole state spaces. \todo{} In fact, they can implicitly \textbf{model} the whole solution space given infinite samplers. However, they are not efficient in the high-dimensional trajectory space. On the other hand, gradient-based methods, including the bunch of works in trajectory optimization, optimize deterministic policies by descending along the local gradient direction. They exploit the convexity of the loss landscape, allowing them to converge to local minima quickly.

There are methods using gradients to optimize distributional policies together. [FIGURE HERE] One can embed gradient descent in population-based methods to achieve a faster convergence speed~[CITE]. However, population-based methods are usually expensive and can hardly share knowledge across agents. Another way is to add random noises sampled from a fixed noise distribution, e.g., Gaussian, to turn a deterministic policy into a stochastic policy and optimize them through gradients~\citep{heess2015learning}. Such first-order gradient estimators are biased under discontinuities as demonstrated in \cite{suh2022differentiable}. Besides, unlike REINFORCE in a discrete environment, Gaussian perturbations in continuous action space are not always useful to help policies escape local minima as it can only model single modality policies. Such methods have become popular in deep reinforcement learning algorithms~[CITE] regardless of these defects. However, it is yet under-developed due to the lack of a differentiable environment.

In this work, we study a generalization of the reparameterization trick~\citep{kingma2013auto}. [FIGURE HERE] We propose to model policy by reparameterizing latent distributions. The latent distributions behave like a sampling-based method, followed by the reparameterization part that maps random samples into an executable action. 
We find that reparameterization provides a unified perspective for some previous sampling and optimization methods. For example, we can view the population-based method as the combination of a categorical distribution represented by the population and then a differentiable policy determined by samples. Similarly, Gaussian policies turn random noises sampled from the fixed standard Gaussian distribution into action through a linear transformation outputted by the network. 
We call it reparameterization, also reminiscent of the differentiable geometry.


We derive a reparameterized policy gradient theorem that optimizes our reparameterized policy. Our theorem in Equation~\ref{eq:rpg_1} generates policy gradients with two parts,
\begin{equation}
    \nabla_{\theta} E_z[R(\tau_\theta(z))]=\int_z p_{\theta}(z|\tau)\left[\underbrace{R(\tau_{\theta}(z))\nabla_{\theta} \log p_{\theta}(z|\tau) }_{\text{REINFORCE}} + \underbrace{\nabla_\theta R(\tau_{\theta}(z))}_{\text{Gradient}} \right] dz. \label{eq:rpg_1}
\end{equation}
The first part estimates gradients through a sampling-based approach like REINFORCE, allowing policies to do random exploration. In contrast, if the environment is differentiable, the second part may optimize the policy directly through gradient descent, enabling a fast convergence speed. The theorem can be viewed as an instance of the stochastic computation graph~\citep{schulman2015gradient, weber2019credit}. Still, we emphasize that first, our formulation is sufficient to cover common sequential decision-making, and second, the existence of the first order policy gradient estimator is related to the problem of differentiation under the integration sign~[CITE][FIGURE HERE] and could be guaranteed by a generalization of the Leibniz integral rule under certain continuous and convergence conditions. Inspired by \cite{suh2022differentiable}, we identify some sufficient conditions for the theorem to hold in both finite horizon trajectory optimization and infinite horizon reinforcement learning. Under mild conditions, we show that our policy reparameterization can help the gradients avoid discontinuities or prevent gradients from exploding.

The theorem motivates us to propose a novel reinforcement learning framework. We discover that our policy reparameterization allows us to represent the multi-modality posterior of trajectories after choosing proper priors.
Using the variational method as shown in Equation~\ref{eq:elbo_1},
\begin{equation}
\log p(O)\ge E_{z\sim \pi_{\theta}} \left[\underbrace{\log p(O|\tau)}_{\text{reward}} + \underbrace{\log p_{\phi}(z|\tau)}_{\text{mutual information}} + \underbrace{\log p(\tau)}_{\text{prior}} \underbrace{-\log \pi_{\theta}(z)}_{\text{entropy}}\right]\label{eq:elbo_1}
\end{equation}
we can approximate the posterior using the latent space in a tractable way, allowing us to explore the global space [FIGURE].
The mutual information term is essential which prevents policies from mode collapse. Our framework naturally optimizes the optimal trajectories' evidence lower bound (ELBO) with hidden variables. One can derive a kind of hierarchical reinforcement learning algorithm or skill learning method based on our formulations. However, they are only a special form of the prior distribution, and our ELBO bound suggests a more general framework.

The advantages of our approach are multi-faceted. The flexibility of reparameterization allows us to model multi-modal trajectory distributions or policies with complex latent structures. These latent distributions could simultaneously search over local minima or help the gradients avoid discontinuities or chaos.
Our method enjoys both the strong exploration ability of sampling and the fast convergence speed of the optimization. 
%Besides, the variational method we used shows how to combine modeling and optimization.
We can also add additional prior constraints through both the hidden distribution's structure and the mutual information term, enabling injecting effective human/data priors.
This work proposes a new algorithm and reveals the relations among sampling (RL), optimization, and probabilistic inference. We hope to provide a unified perspective for general readers and inspire future research.

==> text/legacy_mb.tex <==
\section{Pratical Algorithms}
\subsection{Fixed Horizon Forward Model-Learning}
Let $l_i$ be a series of latent variables that encodes the state $s_i$, and let $H$ be the planning horizon (in the latent space). For a horizon start from $t=nH+1, z_n$ let $I_n=\{t\le i< t+H\}$, $\mathbf{l}_n=\{l_i\}_{i\in I_n}, \mathbf{a}_n=\{a_i\}_{i\in I_n}$ and \textit{next state} $\mathbf{s}_n=\{s_{i+1}\}_{i\in I_n}$, define the joint distribution for hidden planning
$$q_\theta(z_n, \mathbf{l}_n, \mathbf{a}_n|s_{t}, z_{n-1})
= q_\theta(z_n|s_t, z_{n-1})q_\theta(l_t|s_t, z_n)\prod_{i\in I_n}q_\theta(a_i|l_i, z_n)\prod_{i\in I_n/\{t+H-1\}}q_\theta(l_{i+1}|l_i, a_i, z_n) 
$$
and the dynamics
$$p(\mathbf{s}_n|s_t, \mathbf{a_n})=\prod_{i\in I_n}p(s_{i+1}|s_i, a_i)$$
and we define
$$
q_\theta(z, \tau)=p(s_1)\prod_{n\in \{0, 1, 2, \dots\}}q_\theta(z_n, \mathbf{l}_n, \mathbf{a_n}|s_{nH+1}, z_{n-1})p(\mathbf{s}_n|s_{nH+1}, \mathbf{a}_n)
$$

We can now define the encoder for latent variables per short horizon as a state encoder
$$p_\phi(z_n, l_n|\tau)=p_\phi(z_n|\tau)\prod_{i\in I_n} p_\phi(l_i|s_i, z_n).$$

Replace the above $q_\theta, p_\phi$ into our $\RELBO$, we obtain a part for $l_i$
$$\sum_{n\in \{0, 1, 2,\dots\}}\left(-\log q_\theta(l_{nH+1}|s_{nH+1}, z_n) - \sum_{i\in I_n/\{(n+1)H\}}\log q_\theta(l_{i+1}|l_i,a_i,z_n)+\sum_{i\in I_n}\log p_\phi(l_i|s_i, z_n)\right),$$
This requires that we can identify $l_i$ for $s_i$ while maximizing the entropy of $l_{i+1}$, similarly to the variational autoencoder, and we should achieve a high reward. 
Jointly we can view it as maximizing the negative KL divergence between $q_\theta(l)$ and $p_\phi(l_i)$.
Anyway, this forms a very complicated optimization objective.

The common practice of the model-based RL is achieved by constructing a special $p_\phi(l_i|s_i, z_i) \propto e^{-\Vert p_\phi(l_i, z_n)-s_i\Vert^2/C}$ to approximate $p_\theta(l|\tau)$. However, the normalizing factor should sample overall $l_i$, which is intractable.

\subsection{Latent Planning}
Viewing latent planning as a series of latent variables is even possible. Any process that samples latent $\mathbf{l}_n$ that can be identified/interpreted by past and future trajectories can be used.

Planning can be viewed as a sequence of the conditional generative process. However, assume that we have sampled $a'_1, a'_2, a'_3$ from known prior distributions and generate a distribution based on their guessed Q function with the following $p(a|r(a'_1), r(a'_2), r(a'_3))$. Given $a'_1$ execute, we can only infer that $a'_2$ and $a'_3$ may have a lower reward than $a'_1$.

\subsection{Diffusion}
The better practice, instead, we can first project the short $\tau_n$ into low-dimensional trajectory space using something like $p_\phi$ and run a diffusion process to $\mathbf{l}_n$. We need to adjust the feature space to enable high rewards.

Considering the trajectory generative modeling tasks, let the encoder be $p_\phi(x_{0:T}|\tau)=p_\phi(x_0|\tau) \prod_{t=1}^T p(x_t|x_{t-1}, x_0)$ where $p(x_T)$ will be approximately a Gaussian distribution and $p(x_t|x_{t-1}, x_0)$ is also a non-parameterized Gaussian.

We want to approximate the joint distribution of $q_\theta(\tau, x_T)=q_\theta(\tau|x_0)p(x_T)\prod_{t=1}^{T}q_\theta(x_{t-1}|x_t)$ where $q_\theta(x_{t-1}|x_t)$ is an arbitrary neural networks (though it may have an objective to first predict $x_0$ and then sample something).

The objective is to maximize the ELBO
\begin{align*}
\log p(\tau) &\ge E_{x_{0:T}\sim p_\phi}[\log q_\theta(\tau, x_{0:T})- \log p_\phi(x_{0:T}|\tau)]\\&=E_{x_{0:T}\sim p_\phi}[\log q_\theta(\tau|x_0)  + \sum_{t=1}^T\log q_\theta(x_{t-1}|x_t) +\log p(x_T) - \log p_\phi(x_0|\tau) -\sum_{t=1}^T\log p(x_t|x_{t-1})].
\end{align*}
Optimizing $q_\theta$ is usual. The major problem is that the optimization of $p_\phi(x_0|\tau)$ and $\log p_\phi(\tau|x_0)$. Through the reparameterization trick, we can optimize $p_{\phi}$ by optimizing $p_\phi(x_0|\tau)$ and the gradient of $x_0$ through the reparameterization trick. The gradient of $x_0$ however, is related to $q_\theta(\tau|x_0)$, and the gradient of $\log q_\theta(x_{t-1}|x_t)$, which can be approximated by its expectation.

The backpropagation is very tricky. Assuming the computation of $\partial x_t/\partial x_0$ is easy to compute when $x_0$ is fixed, we then need compute the gradients of $\frac{\partial q_\theta(x_t|x_{t-1})}{\partial x_t}$ and $\frac{\partial q_\theta(x_t|x_{t-1})}{\partial x_{t-1}}$, this is however, possible. Related here ~\url{https://openreview.net/pdf?id=DoGRjqtgjph}.

A PPO-like trick to bound the offline optimization might be useful here. 

\subsection{Proximal Policy Optimization}
Let me use a $z_n$ for every $H$ steps so that we can easily extend the single sample example to multiple samples. 
We can always introduce a diffusion process on learned functions on the low-dimensional trajectory space so we can talk about it later. Each $H$ step can be differentiable or not, but we will not differentiate them among different stages. If we need to do so, we rely on a value network or a differentiable Q value.

Let me first ignore gradients and assume that we have stages with ending values. Thus we have two value networks $V(s_i, z_n)$ and $V(s_i, z_{n-1})$ where $nH+1\le i\le (n+1)H$ are baselines. The clipped reward is standard. In each/or several PPO updates, we update the encoders. We will update the input to $z$ and the inputs for $s$ separately.

\textbf{Model-based version with latent action gradients}
We reintroduce $\mathbf{x}_n$, the latent dynamics model that can be learned with the $\RELBO$ directly. To avoid the strange normalization of the reconstruction loss, we project the states into a latent space through a variational auto-encoder trained on the PPO buffer of recent trajectories/states seen so far.

We then apply a diffusion model to build our encoders and train a decoder to reconstruct the trajectories and optimize both the latent variables, the VAE encoder, and the actions with (gradients).

The sampling process is $z_n, x_0$ by reverse diffusion that generates the embedding of $\mathbf{a}_n, \mathbf{s}_n$ in the end. [ensuring the reconstruction.]

Then constrained by the divergence of the dynamics, optimize the action components...

We first train the reverse diffusion methods to ensure that the diffusion process can reconstruct the original feature anyway by minimizing the KL divergence in a very strange way.

When there is no gradient, we can optimize $a_n$ and clip its gradient if it has deviated too much.

Except for $z_n, x_0$, the remaining part is deterministic and can be optimized by the given differentiable reward directly ($\RELBO$ contains the known rewards and the latest value, the log probabilities of the latent, the encoder, and the prior.).
The training of $z_n$ and $x_0$ can be done by sampling directly. In this case, it's better to optimize the policy with constrained optimization methods directly. 

==> text/motivation.tex <==
\section{Motivation}
% Reparameterization and Policy Optimization
% Expanded intro. 

%First is the lack of multimodal. 
%Generalized Reparameterization to represent multi-modal.
%In the finite horizon, many things could be viewed as a kind of reparameterized policy.
%Mention that many things could be changed. 

% Combine REINFORCE to select multi-modal.
%However, the high-level distribution is not differentiable ——  study.




%Given a differentiable MDP, a neural network is a differentiable map from the random noises into sampled trajectories of the MDP, which forms the manifold of the policy space. In REINFORCE, we need to compute the gradients of the path integral, which follows the Leibniz integral rule  
%\href{https://www.math.ucla.edu/~tao/preprints/forms.pdf}{forms}
%$$\left.\frac{d}{dt}\right|_{t=0}\int_{\text{im}_{\psi_t}(\Omega)}\omega=\int_{\Omega}\mathcal{L}_{\Psi}\omega.$$
%Here, we only consider the finite horizon trajectory optimization case to simplify the analysis\footnote{Not only because we do not need to consider limitation, but also we can compute value gradients easily without taking special care of the discount factor.}.
% Here we illustrate the idea of reparameterized policy and its gradient. To illustrate the purpose, in this section, we assume that we can sample random noises in advance and then rollout the whole \textbf{finite horizon} trajectories. This makes the problem similar to the continuous bandit, and we can analyze the gradients easily without worrying too much about their convergence. See Equation. %~\ref{eq:rpg_1}.

%\todo{A formal description of the finite horizon and discrete cases. The proof for the general cases will be put in the appendix.}
%Let's consider the path integral problem. Let $z=f_\theta(s, \xi)$ be a non-differentiable function $\rightarrow z\sim p_{\theta}(z|s)$ and $a=g_\theta(s, z)$ be the action sequence. The dynamics function will return a state $s'=T(s, a)$ and reward $r(s, a)$. For deterministic action $a=g_{\theta}(s, z)$, the following policy gradient theorem holds 
%$$\nabla_{\theta} E[R(a)]=\int_z p_{\theta}(z|s)\left[\nabla_{\theta} \log p_{\theta}(z|s) r(s, g_{\theta}(s, z)) + \nabla_\theta r(s, g_{\theta}(s, z)) \right] dz.$$




==> text/pathological_case.tex <==
\section{Proof of the Reparameterized Policy Gradient Theorem}

% When we use the path-wise gradients to estimate the policy gradient of the expectation, it is not always feasible to swap differentiation and integration in the following equations,
% \begin{align*}
%     \nabla_{\theta} \E[\RELBOTAU]
%     &=\textcolor{red}{\nabla_{\theta}} \int_{z} \QTHETA\RELBOTAU d z =\int_{z}\textcolor{red}{\nabla_{\theta}} \left( \QTHETA\RELBOTAU\right) d z 
% \end{align*}
%Thus, we can sample trajectories and use the first-order gradient to update the policy parameter $\theta$. However, before 
%As demonstrated by ~\citep{suh2022differentiable} and ~\citep{li2018differentiable}, the above equality may suffer from the issue of discontinuities. When the reward landscape has discontinuous points, there will be a bias caused by the motion of the discontinuity as suggested by the Leibniz integral rule. We refer interested readers to Appendix~\ref{appendix:bias1d} for a detailed illustration of the difference between the zeroth-order gradient estimate and the first-order gradient estimate under the expectation we do not find in the literature.

%We now state a policy gradient theorem under several regularity conditions. The major requirement is the Lipschitz continuity of the whole system. Note that we do not ask for the continuity of the neural networks and support functions such as ReLU.
\subsection{Regularity Conditions}
\label{sec:regularity_conditions}

%Let $\mathcal{Z, S, A}$ be open sets.
%Let $\mathcal{Z}$ be a measure space, and $\theta$ belongs to an open set. 
Let $\theta\in \Theta=(-\epsilon, \epsilon)\in \mathbb{R}$ without loss of generality and $\Omega=\{z\in \mathcal{Z}|\QTHETA>0\}$ be a measure space, then for $z\in \Omega, \theta\in [-\epsilon, \epsilon]$, we make the following assumptions
\begin{assumption}[Bounded ELBO]
The reward $R$, prior density $\log p(\tau),\log q_\theta(z|\tau), \log p_\phi(z|\tau)$ are bounded for all $\tau$.\label{assumption:bound}
\end{assumption}
\begin{assumption}[Lipschitz Condition]
$q_\theta(z|\tau)$, $ \log q_\theta(z|\tau), \log p_\phi(z|\tau)$, prior distribution $\log p(\tau)$, action policy $\mathbf{f}_\theta(s_t, z, t)$, reward $R$ and dynamics $h(a_t, s_t)$ are Lipschitz continuous w.r.t. any $s, a$ and continuous $z$. In addition, $q_\theta$ is Lipschitz continuous w.r.t. $\theta$. \label{assumption:lipschitz}
\end{assumption}
\begin{assumption}[Lebesgue-integrable]
The probability density $\QTHETA$ and its derivative $|\nabla_\theta \QTHETA|$ is Lebesgue-integrable jointly over $\Omega$ and their integration is bounded for all $\theta\in [-\epsilon, \epsilon]$.\label{assumption:lebesgue}
\end{assumption}
%\begin{assumption}[Dominated Convergence]
%There is a Lebesgue-integrable function $g(z):\mathcal{Z}\rightarrow \mathbb{R}$ such that $\nabla_{\theta}q_\theta$ for all $x\in X$.
%\end{assumption}

%Notice that the Assumption~\ref{assumption:bound} and \ref{assumption:lipschitz} should be guaranteed by the design of the reward and  function approximator. 
Assumption~\ref{assumption:bound} is easy to guarantee when the state space and the action space are compact and the time horizon $T$ is finite because continuous functions on a compact set are always bounded.  Similarly, for bounded inputs, the common neural networks can also satisfy Assumption~\ref{assumption:lipschitz}. Otherwise, we can simply clamp them before feeding them into a neural network to make the input bounded, as we do not need the network and the environment to be continuously differentiable as in Lemma~\ref{lemma:leibniz_general_form} but only absolutely continuous.
We require the dynamics $h(a_t, s_t)$ to be Lipschitz continuous, ruling out chaotic systems. %similarly to the requirements in Picard–Lindelöf theorem~[CITE].  

Assumption~\ref{assumption:lebesgue} holds for common distributions. For example, given a Gaussian distribution $p(z)=e^{(-z^2/(2 \sigma^2))}/(\sqrt{2 \pi} \sigma)$, the parameter $\sigma$'s partial derivative $\frac{\partial p}{\partial \sigma}(z)=e^{(-z^2/(2 \sigma^2))} (-\sigma^2 + z^2)/(\sqrt{2 \pi} \sigma^4)$ is simply a function of exponential family and can be verified to be absolutely integrable on $\mathbb{R}$ and bounded for any domain $\sigma\in [a,b], a, b>0$.


\subsection{Proof of Theorem \ref{theorem:RPG}}
To differentiate under integration, we use the following Lemma~\citep{planet_libniz, l1995note}, 
%or \href{https://encyclopediaofmath.org/wiki/Parameter-dependent_integral}{here} [CITE].
\begin{lemma}[Leibniz integral rule] Let $X$ be an open subset of $\mathbb{R}$, and $\Omega$ be a measure space. Suppose that a function $f: X\times \Omega\rightarrow \mathbb{R}$ satisfies the following conditions:
\begin{enumerate}
    \item $f(x, \omega)$ is a measurable function of $x$ and $\omega$ jointly and is integrable over $\omega$ for almost all $x\in X$ fixed.
    \item For almost all $\omega \in \Omega$, $f(x, \omega)$ is an absolutely continuous function of $x$ (the derivative $\partial f(x, \omega)/\partial x$ exists almost everywhere).
    \item $\partial f/\partial x$ is ``locally integrable'', that is, for all compact intevals $[a, b]\in X$,
        $$\int_a^b\int_\Omega\left|\frac{\partial }{\partial x}f(x, \omega)\right|d\omega dx <\infty.$$
\end{enumerate}
\label{lemma:leibniz}
Then for almost every $x\in X$, its derivative exists and $$\frac{d}{dx}\int_{\Omega}f(x, \omega)d\omega=\int_\Omega\frac{\partial }{\partial x}f(x, \omega)d\omega$$
\end{lemma}

Then it is easy to prove Theorem~\ref{theorem:RPG}.
\label{sec:proof_of_RPG}
\begin{proof}
%To apply Lemma~\ref{lemma:leibniz}, we need to show that under the assumptions, the function $q_\theta(z|s_1)\RELBOTAU$ is a Lipchitz function, and its gradient is dominated by an absolutely integrable function.

% DO  we need to make q_\theta(z|s_1) lipschitz continous to make this hold?
%, as it can be written as a countable union of $\{z\in \mathcal{Z}|q_\theta(z|s_1)>1/n\}, \forall n\ge 1$ as $q_\theta(z|s_1)\in L^1$. [NOT SURE IF THIS IS CORRECT].

Define the measurable function $f(\theta, z) = \QTHETA\RELBOTAU$.

Since $\RELBOTAU$ is bounded by a constant $M$ by Assumption~\ref{assumption:bound} and $\QTHETA$ is positive and Lebesgue-integrable by Assumption~\ref{assumption:lebesgue}, their product's absolute value will be bounded by $\QTHETA M$, so $f(\theta, z)$ becomes Lebesgue-integrable for every $\theta$.

By Assumption~\ref{assumption:lipschitz} and assuming the horizon is finite, the trajectory $\tau$ will become a Lipschitz function with respect to $\theta$ and $z$, so as $\RELBOTAU$, $\QTHETA$ and their products $f(\theta, z)$. Thus $\frac{\partial f(\theta, z)}{\partial \theta}$ exists almost everywhere for all $z\in \Omega$.

To bound its derivative, let $\RELBOTAU$ be $L$-Lipschitz w.r.t. $\theta$, notice that 
$$
|\nabla_\theta f(\theta, z)|=\left|\RELBOTAU\nabla_{\theta}\QTHETA  +  \QTHETA\nabla_{\theta} \RELBOTAU\right|
\le M\left|\nabla_\theta \QTHETA\right| + L \left|\QTHETA \right|,
$$
is dominated by the sum of two Lebesgue-integrable functions  whose integration is bounded for all $\theta\in \Theta$ by Assumption~\ref{assumption:lebesgue}. Thus its gradient must be locally integrable. Then applying Lemma~\ref{lemma:leibniz}, we can do differentiation under the integration sign and finish the proof as  
\begin{align*}
    \nabla_{\theta} E[\RELBOTAU]
    &=\int_{z}\nabla_{\theta} \left( \QTHETA\RELBOTAU\right) d z 
    \\
    &=\int_{z}\RELBOTAU\nabla_{\theta}\QTHETA(z|s_1) + \QTHETA\nabla_{\theta} \RELBOTAU dz\\
     &=\int_{z} \QTHETA\left[\RELBOTAU\nabla_{\theta} \log \QTHETA +\nabla_\theta \RELBOTAU \right] d z. 
\end{align*}
\end{proof}

We want to emphasize the importance of the Lipschitz continuity that helps to bound the integration. Informally, the Lipschitz condition is directly related to the scale of the path-wise gradient. When the Lipschitz constant is too large, the environments will generate exploding gradients~\cite{} or contains sharp changes in the reward landscape, similarly to the discontinuity and causing empirical bias~\cite{suh2022differentiable}.
Besides, when the reward landscape has discontinuous points, there will be a bias caused by the motion of the discontinuity, as suggested by the Leibniz integral rule. We refer interested readers to Appendix~\ref{appendix:bias1d} for a detailed illustration of the difference between the zeroth-order gradient estimate and the first-order gradient estimate under the expectation we do not find in the literature. Note that we do not ask for the continuity of the gradients and support activation functions such as ReLU.

The finite horizon assumption is also necessary to make the theorem holds, otherwise the gradients $\nabla_\theta \RELBOTAU$  may be unbounded if we do not set up a suitable discount factor. %We leave the rigorous discussion as future work.


% \section{Discussion on Future Works}
% Pathological Cases
% \subsection{How to avoid discontinuities}
% Rather than running policy and then adding noise, we prefer sampling first and then doing optimization.  For continuous $z$, if we are able to make the function value vanish at the boundary, everything will be ok. This should be true as the robust policy does not have to be on the decision boundary and thus $p_{\theta}(z|s)$ will be zero.

% \todo{Replace $C^1$ to Lipschitz continuous.}
% \begin{theorem}
% Let $z\in R^n$, $p(z)\in C^1$, $p(z)\ge 0, \int p(z) dz=1$. $f(z)$ is bounded and $C^1$ at any $\{z|p(z)>0\}$, then $p(z)f(z)$ is continuous and differentiable and integrable.
% \end{theorem}

% \begin{proof}
% The integrability is obvious as $f(z)$ is bounded and $p(z)$ is absolutely integrable. To prove the differentiablity, For $p(z)>0,$ since $f(z)$ is differentiable, $p(z)f(z)$ must be differentiable. Then for any $p(z_0)=0$, since $p(z)\ge 0$, we must have $ p'(z_0)=0\Rightarrow p(z)=p(z_0)+p'(z_0)(z-z_0)+o((z-z_0)^2)=o((z-z_0)^2)\Rightarrow \lim_{z\rightarrow z_0}(f(z)p(z)-p(z_0)f(z_0))/(z-z_0)=\lim_{z\rightarrow z_0}o((z-z_0)^2)f(z)/(z-z_0)=0$ for any bounded $f(z)$, which means $p(z)f(z)$ is differentiable at $z_0$ and has gradients $0$.  
% \end{proof}


% \hza{The major concern is that even we can compute the gradients, if the method with an improper initialization can help the gradient to go across the non-continuous/or non-convex region is unknown. This would happen even for continuous environment with good gradients.. Question: can we ensure the entropy with infogail in non-differentiable envs given that $p_{\phi}$ is always differentiable to the action $a$?}

% \subsection{Controllability for Chaos}


\section{Learning a differentiable world model}
\subsection{Method}

\begin{algorithm}[!htp]
	\caption{Model-based \fullname{}}
	\begin{algorithmic}[1]
		\State\textbf{Input:}  $p_\phi, \pi_\theta, h_\psi, R_\psi, f_\psi, Q_\psi$
		%\State Initialize $p_\phi, \pi_\theta$, construct the replay buffer $\mathcal{B}$.
		\While {time remains}
                \State Sample start state $o_1$ and encode it as $f_\psi(o_1)$. Select $z$ from $\pi_\theta(z|s_1)$.
                \State Execute the policy $\pi(a|s, z)$ and store transitions into the replay buffer $\mathcal{B}$.
                \State Sample a batch of trajectory segment of length $K$ $\{\tau^i_{t:t+K}, z\}$ from the buffer $\mathcal{B}$.
                \State Optimize $\psi$ using Equation $\ref{eq:mb_dyna}$.
                \State Optimize $\pi_{\theta}(a|s, z)$ with gradient descent to maxmize the value estimate in Equation $\ref{eq:mb_value}$ for $s, z$ sampled from the buffer.
                \State Optimize $\pi_{\theta}(z|s_1)$ with policy gradient to maximize $V_{\text{estimate}}(s_1, z)-\alpha \log \pi_{\theta}(z|s_1)$ for $s_1$ is sampled from the buffer.
                \State Optimize $\phi, \alpha, \beta$ and other auxiliary networks.
		\EndWhile
	\end{algorithmic}
	\label{algo:mbrpg}
\end{algorithm}

\subsection{Experiment}
We first compare our method with SAC~\cite{haarnoja2018soft} on locomotion tasks (Cheetah-v3 and Humanoid-v3 in OpenAI Gym~\cite{brockman2016openai}) in Figure~\ref{fig:mbrl_curve}(a) and (b). We plot the learning curve of MBRPG together with the SAC's performance after training for 3 million steps. We can see that by learning the model, our method achieves on-par performance with fewer samples. In particular, our method only requires $1$ million samples to reach $15000$ scores on Cheetah-v3 and only $0.5$ million samples to reach $6000+$ scores on Humanoid-v3. This attributes to the efficiency brought by learning a model for policy optimization. However, we observed that removing the latent variables and the variational bound, which is a baseline model-based RL algorithm (MBRL), did not affect the performance of our method. We conjecture that these locomotion tasks do not require a multi-modal policy for exploration, and a Gaussian policy is sufficient.

To illustrate the effectiveness of our approach, we have built two environments that need multi-modality explorations, as illustrated in Figure~\ref{fig:mbrl_env}. In (a) AntMove environments, an ant robot can move either upward or rightward to reach one of the two goal regions represented by the black circle. The agent always receives a penalty proportional to its distance to the closest goal, which motivates it to go upward instead of moving right. However, if the agent chooses the longer right path, it will receive a higher bonus when it reaches the goal. Such a local optimum will trap a single modality agent, as shown in Figure~\ref{fig:mbrl_curve} (c). When we remove the latent space and the latent policy $p(z|s_1)$, the baseline single-modal RL policy (MBRL) will get stuck in the local optima, while our approach (MBRPG), thanks to its ability to maintain multi-modality trajectory distribution, will attempt to go right even when it is sub-optimal at the beginning and thus has a higher chance to find the global optima. We also test our method for an $11-dof$ mobile robot for opening the cabinet shown in Figure~\ref{fig:mbrl_env} (b). It is easier for the robot to open the left door, but it will receive a higher reward when it opens the right one. Similarly, the normal RL agent modeled by a Gaussian distribution (MBRL) fails to explore a way to open the right door. In contrast, our method explores the two directions simultaneously and can open the right one, in the end, resulting in higher rewards, as shown in Figure~\ref{fig:mbrl_curve}.

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figure/mbrl_env.png}
    \caption{Non-differentiable environments}
    \label{fig:mbrl_env}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figure/mbrl.png}
    \caption{Experiments with a learned world model.}
    \label{fig:mbrl_curve}
\end{figure}



\section{Ablation Studies}

In this section, we first study the importance of the trajectory encoder to understand what role it plays in helping maintain a multi-modality trajectory distribution. Then, we show how hyperparameter controlling the reward weight of entropy of action affects algorithms that have different policy paramterization.

\begin{figure}[h]
    \begin{subfigure}[b]{1\textwidth}
    % \centering
    % \includegraphics[width=1\textwidth]{figure/env_thumbnail.png}
    \includegraphics[width=1\textwidth]{figure/numerical_ablation_exp.png}
    \includegraphics[width=1\textwidth]{figure/numerical_ablation_exp_legends.png}
     %\label{fig:envs}
    \end{subfigure}
    \caption{Ablating trajectory encoder}
    \label{fig:ablation_encoder}
\end{figure}

In Figure \ref{fig:ablation_encoder}, we show the importance of the trajectory encoder, We can see that when we do not optimize the mutual information between $z$ and $\tau$ through $\log p_\phi(z|\tau)$ (Ours (no info loss)), our method degrades to almost identical behavior as Adam. We can see that the best-performing method is our method in its current form.

% \begin{figure}[h]
%     \begin{subfigure}[b]{1\textwidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{figure/env_thumbnail.png}
%     \includegraphics[width=1\textwidth]{figure/ablate_ent_a_banditx.png}
%     \includegraphics[width=1\textwidth]{figure/ablate_ent_a_banditx_legends.png}
%      %\label{fig:envs}
%     \end{subfigure}
%     \caption{Experiment result after ablating entropy weight.}
%     \label{fig:bandit_enta_exp}
% \end{figure}

% In Figure \ref{fig:bandit_enta_exp}, we varied the reward weight (abbreviated as ``enta'') of $-\log\pi(a)$ to control the initial standard deviation of the Gaussian policy under the maximum entropy framework. Results are shown in Figure \ref{fig:bandit_enta_exp}. The largest ``enta'' is deliberately selected to stall all algorithms. Then we vary ``enta'' and run all algorithms with linear reward weight annealing similar to Figure~\ref{fig:reward_after_gaus_filter}. We can see no matter how gradually we decreased the standard deviation by changing ``enta'', no variation of REINFORCE or Adam successfully solves the task. When the standard deviation is large enough, our method is also affected by similar issue as Adam, as all modes have too large standard deviation that covers both modes, causing the expected gradient to be positive for all modes of policy. Using a zeroth order estimator like reinforce to optimize ELBO for our method instead of a first order method helps with the performance.

% \section{Other stuff}
% To understand why single modality policy fails to deliver the promise, and how a multi-modality policy is able to achieve the desired behavior, we visualize the reward landscape after it's passed through a Gaussian filter in Figure \ref{fig:reward_after_gaus_filter} with standard deviation gradually decreased from left to right, which is equivalent to the landscape of expected reward of the mean $\mu(\theta)$ of the single modality Gaussian policy during training (assuming a similar strategy of decreasing standard deviation is applied). Here the red dotted line is at the argmax of expected reward. In other words, if a single modality policy like Gaussian is used, the ideally optimal $\mu(\theta)$ should be at the red dotted line after each time the standard deviation is decreased. However, the global maximum of the expected reward landscape after decreasing the standard deviation changes drastically from the right mode to left mode. This behavior will devastate all gradient based algorithms optimizing a single modal policy. To study this effect, we ablate the components of the algorithm, the hyperparameters of the algorithms, and the hyperparameters of the environment separately to understand how the decreasing standard deviation and the shape of reward landscape play a role during training.

% \begin{figure}[h]
%     \begin{subfigure}[b]{1\textwidth}
%     % \centering
%     % \includegraphics[width=1\textwidth]{figure/env_thumbnail.png}
%     \includegraphics[width=1\textwidth]{figure/ablate_env_rdscale_banditx.png}
%     \includegraphics[width=1\textwidth]{figure/ablate_env_rdscale_banditx_legends.png}
%      %\label{fig:envs}
%     \end{subfigure}
%     \caption{Environment after ablating the right mode area and experiment results.}
%     \label{fig:bandit_area_exp}
% \end{figure}

% In Figure \ref{fig:bandit_area_exp}, we varied the area of the right reward mode of Bandit 1 while fixing the left mode with area of 0.36. We run variations of our algorithm on it. To ensure the comparison is fair, we set the standard deviation scale and reward weight of action entropy (enta) to be the same for all algorithms. The enta hyperparameter is set to be large enough so that all action distributions are initialized to be indistinguishable from a uniform distribution in the action, and at the same time small enough such that all the algorithms can at least learn something. We then anneal the reward weight up linearly with identical rate for all algorithms until experiment is finished. 

% We can see that only optimizing a single modality policy like Reinforce is very sensitive to the expected reward during annealing. At some point during training, the gradually decreasing standard deviation can no longer cover both modes. To optimize expected reward, the mode collapses on the mode with larger expected reward, not necessarily the mode that contains globally optimal solution. When the area of right mode is smaller than the left, reinforce can find the left mode by gradually decrease the standard deviation, and vice-versa when the area of right mode is larger. For Adam, initializing with a large standard deviation does not work. When the actions are sampled near uniformly on the action space, the gradient of policy mean with respect to average reward is always positive. After the mode arrives at the discontinuity on the right, the gradient will continue to be positive, no matter how standard deviation is being tuned. For our methods, both using (Ours) or not using path-wise gradient (Ours (Reinforce)) eventually finds the globally optimal solution, with the latter one being slower.



==> text/reproducibility_statement.tex <==
\section*{Reproduciblity Statement}
% It is important that the work published in ICLR is reproducible. Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. For example, for novel models or algorithms, a link to a anonymous downloadable source code can be submitted as supplementary materials; for theoretical results, clear explanations of any assumptions and a complete proof of the claims can be included in the appendix; for any datasets used in the experiments, a complete description of the data processing steps can be provided in the supplementary materials. Each of the above are examples of things that can be referenced in the reproducibility statement. This optional reproducibility statement will not count toward the page limit, but should not be more than 1 page.

We will provide an open-source implementation of our method on GitHub. We will also update more illustrative examples and demos to our \href{https://sites.google.com/view/iclr2023vrpl}{website}. The hyperparameter used in the experiment section can be found in Table \ref{tab:hyperparams} in the appendix. The theoretical results are also in multiple sections of our appendix.

==> text/todo.tex <==
\section{\todo{}}


\paragraph{Remark}
After ensuring the existence of the gradients and value gradients, we can now come back to the common statement of the policy gradient theorem. We can define the $Q$ function, thus 
$$Q^{\pi_\theta}(z, s)=R(s, g_{\theta}(s, z), z)+V^{\pi_{\theta}}(f(s, g_{\theta}(s, z), z), z)$$
$$\nabla_{\theta} Q^{\pi_\theta}(z, s)=\nabla_{\theta} R(s, g_{\theta}(s, z), z) +\nabla_{\theta} V^{\pi_{\theta}}(f(s,g_{\theta}(s, z), z),z)$$
$$\nabla_{s} Q^{\pi_\theta}(z, s)=\nabla_{s} R(s, g_{\theta}(s, z), z) +\nabla_{s} V^{\pi_{\theta}}(f(s,g_{\theta}(s, z), z),z)$$
$$\nabla_{s,\theta} V^{\pi_{\theta}}(s, z)=\int_{z'}\pi_{\theta}(z'|s, z)\left[\nabla_{s, \theta} \log \pi_{\theta}(z'|s, z)Q^{\pi_{\theta}}(z', s)+\nabla_{s,\theta} Q^{\pi_\theta}(z',s)\right]dz'.$$


In case that the discounted distribution can be unbounded.. $d^{\pi}(s, z|s_0,z_{-1})=\sum_{t=0}^{\infty}\gamma(s_t)d^{\pi}_t(s, z)$, we can rewrite the policy gradient theorem into the familiar form \todo{the policy gradient with discounted distribution}.



\textbf{Tricks for PPO}
We need to learn value $V(s_i, z_i)$, and then we can train the actor part through truncated gradients. No need for GAE.

We require the environment to support the batched version, e.g., run multiple trajectories in parallel and return truncated rewards and information. Then we run in the environments iteratively
\begin{itemize}
    \item For each forward trajectories
        \begin{itemize}
            \item collect $V(s_T, z_T)$.
            \item compute the gradients with the help of the value of the previous episode, also backward the gradients of the hidden $z$ network;
            \item compute the gradient with respect to $\theta$.
        \end{itemize}
    \item Update the policy network;
    \item Update the value network.
\end{itemize}



What we need to do:
\begin{itemize}
    \item Major algorithm components: sequential $z$ \done{Roughly works}; PPO for high-level \done{does not help too much yet}; mixture of Gaussian hidden (so that we can better avoid discontinuities); Barrier to detect discontinuities. Subs:
    \item four major environments: continuous bandit, rigid body push, soft body pinch, \textbf{cut} and maze, \hza{Robot arm for chaotic system}.
    \item The primary message of the experiments:
        \begin{itemize}
            \item our methods enable more global search than pure gradient-based optimization [benefits from the sampling-based method]
            \item faster than pure policy-gradient due to the gradient descent ..
            \item potential to handle non-continuities [key properties to connect both]
            \item useful even in practice by showing its performance on a real physical system.
        \end{itemize}
    \item defense [put them in the supplementary]
        \begin{itemize}
            \item Comparison with adding Gaussian/local noise noise
            \item regarding sequential z: need compare with the population based method. Enable hierarchical (structured) exploration?
            \item Argument for the real-world transfer.
        \end{itemize}
\end{itemize}

Not now:
\begin{itemize}
    \item The verification of the Leibniz integral rule does not seem necessary as it is true for sure, when $p(z)=0$.
    \item Normalizing flow seems too tricky to tune. I will give up it unless someone can figure out its training properties. 
    \item Other potential latent structure, for example, sample $z$ not only according to the current observation, but also the past $z$ to make the exploration more consistent. The sequential $q_{\phi}(z|\tau)$ that conditions on the future information may also help.
    \item Real world robot experiments; execute a plasticine moving task given pointcloud condition or just convincing them with the motion planning tasks that we can then f ollow the planned trajectories in the real world.
    \item  Maybe we can prove that if we can do such decomposition, we can achieve a faster convergence speed. We may need show the convergence bound of policy gradient, gradient descent, and the mixture under certain Lipschitz conditions (or at least illustrate it by experiments).  
    \item Asymptopic optimality. Clearly such kind of optimization is NP-hard as GMM seems to be NP-hard. The question is that if we can find an asymptotic optimality guarantee like $RRT^*$ when we increase the number of $Z$. 
    \item Exploration problems with an decreasing temperature and its connection to statistical physics and quantum physics.
    \item \href{http://www.cs.cmu.edu/~mgormley/courses/10418/slides/lecture26-npbayes-ink2.pdf}{dpmm}
\end{itemize}


Figure:
\begin{itemize}
\item teaser: showing the optimization curve of a local gradient descent; and a trajectory distribution that is optimized jointly.  
\item Idea of combining sample and gradient
    \begin{itemize}
        \item Demonstrate the issue of local minimum and discontinuous of Gaussian policy (reynolds transport theorem)
        \item random samples; inefficiency; and may cover not-good region.
        \item Ours: sample first and then do local optimization. 
    \end{itemize}
\item Better explanation of Reynolds transport theorem.
\item Better explanation of the structured variational inference.
\end{itemize}



\section{Experiment Note}
\begin{itemize}
    \item For rsample, we can not detach the action when computing log prob for entropy.
    \item For sample, we need to make sure that we do not pass the gradient of action through log prob. 
    \item To compute the entropy of the gradient, we only need to compute the first part
        $$\nabla\sum_x  p(x)\log p(x)=\sum_x p(x)(\log p(x)\nabla \log p(x) +\nabla \log p(x))$$
    \item the entropy of a categorical distribution is hard to optimization (it's even not convex when $x$ is very small). The gradients of a sigmoid $\sigma(x)\log \sigma(x) + (1-\sigma(x))\log (1-\sigma(x))$ will decay to $0$ when $x$ approaches  $\infty$ or $-\infty$.
    \item ELBO bounds hold for sure; However, if we use determinstic policy, we have to compute the log prob of the determinsitic policy, which is the dirac delta, not possible in reality..
    \item Near determinisitic policy head, several discrete z, could maximize the entropy (if reward is not the dominate term).
    \item mutual information term is necessary.
    \item uniform distribution prior is not suitable for optimization (especially for gradient-based policy optimizer..); Gaussian prior is better as it is convex.
    \item First order policy estimator can't handle large gradient in some penalty methods .. when std is very large, it can't learn easily with a small batch size.
    \item in trajectory opt, action entropy / reward will dominate the z term..
    \item reward clip seems harmful (hurting symmetry.)
    \item In hierarchical RL (like us), we should not normalize the advantage ..
\end{itemize}


\section{Path integral formulation in the quantum cases}

Feymann..

\section{Relationship with the bellman-equation}
The relationship of the policy gradient and the bellman equation in the sequential case is non-trivial and actually I do not see anyway to let the iterative method natrually emerge. However, we can still follow the Soft Q learning and Schulman's work to make some derivation, in my own way. Let $\pi(a)\propto e^{Q(a)}$, following InfoNCE, we can see that the gradient of the log-propability has a simple form of
\begin{align*}
\nabla \log \pi(a)=\nabla Q(a)-\nabla \log \int_a e^{Q(a)}da=\nabla Q(a)-\frac{\nabla \int e^{Q(a)}da}{Z}\\
=\nabla Q(a)-\int \frac{e^{Q(a)}}{Z}\nabla \log e^{Q(a)}da=\nabla Q(a)-E_{a'\sim \pi}[\nabla Q(a')]
\end{align*}
Thus in policy gradient we have
\begin{align*}\nabla \int \pi(a)R(a)da&=\int \pi(a)\left[\nabla Q(a) - E_{a'\sim \pi}[\nabla Q(a')]\right]R(a)da \\
&=E_{a\sim \pi}[\nabla Q(a)R(a)] - E_{a'\sim \pi}[\nabla Q(a')]\int \pi(a)R(a)da\\&=E_{a\sim \pi}[\nabla Q(a)\left(R(a) - V\right)].
\end{align*}
We can see that the normalizing factor naturally emerges as a value. Note that in general $E_{a\sim \pi}[\nabla Q(a)]\neq 0$. We can not omit the $V$. If we set $R'(a)=Q(a)+\log \pi'(a)-\log \pi(a)$, and notice that $\nabla \int \pi(a)\log \pi(a) da = E_{a\sim \pi}[(\log \pi(a)+1) \nabla \log \pi(a)]$ where the constant $1$ could be eliminated in the policy gradient. We have the new reward $R_{ent}(a)=R(a)-\log\pi(a)+\log p(a)$ and the new value $V_{ent}=\int_a \pi(a)(R(a)+\log p(a)-\log \pi(a))da$. 

Suppose that the soft value $Z=\log \int e^{Q(a')}da'\rightarrow \log \pi(a)=Q(a)-Z\Rightarrow Q(a)=\log \pi(a)+Z\Rightarrow R_{ent}=R(a)-Q(a)+Z.$ %$$R_{ent}(a)-V_{ent}=R(a)-Q(a)+Z +\log p(a) - \int \pi(a') (R(a')+\log p(a')-Q(a')+Z)da'$$
%$$=R(a)-Q(a) +\log p(a) - \int \pi(a') (R(a')-Q(a')+\log p(a'))da'$$
If the prior $p(a)$ is a constant or let $R'=R+\log p(a)\Rightarrow $ the policy gradient becomes
$$E_{a\sim \pi}[\nabla Q(a)(R(a)-Q(a)-E_{a'\sim \pi}[R(a')-Q(a')])].$$
$$=E_{a\sim \pi}[(\nabla\log \pi(a)+\nabla Z) (R(a) - V - Q(a)+E_{a\sim \pi}Q(a))] $$
$$=E_{a\sim \pi}\left[\nabla \log \pi(a)(R(a)-Q(a)+ Z)\right],$$
Here we use the fact that $E_{a\sim \pi}[\nabla \log \pi(a)\cdot \text{constant}]=0$ and $E_{a\sim \pi}[\text{constant}\cdot (Q(a)-E_{a'\sim \pi}Q(a))]=0$. As for the bellman equation as we have:
$$E_{a\sim \pi}[\nabla (\log \pi(a)+Z-R(a))^2]\approx E_{a\sim \pi}[\nabla \log \pi(a)(\log \pi(a)-R(a)) + \nabla Z (Z-(R-\log\pi(a)))]$$
$$=E_{a}[\nabla \log \pi(a) (\log \pi(a)-R(a)) + \nabla (Z-V_{ent})^2]$$

One can see that the two have different terms brought by $-E_{a\sim \pi}[\nabla Q(a)]E_{a'\sim \pi}[R(a')-Q(a')]=\nabla Z (V-\sum_{a}Q(a))$, which is proportional to the approximation error between $V$ and $\sum_{a}Q(a)$.

However, it's not clear why the two will reach the same optimal value with different behavior distribution.
Ideally, we may find a way to bound the differences through the differences between $\pi$ and $\pi'$, and bound the optimality based on the model class. Unfortunately, I do not have enough theoretical tool to characterize these terms. What's worse, it is possible that they not not bounded. Instead, it is highly possible that we can reweight experience through a density model/probabilistic model.

==> variational_inference.tex <==
\begin{itemize}

\item \href{https://arxiv.org/pdf/1805.00909.pdf}{RL as inference} Let $\tau=(s_1,a_1,\dots, a_T, s_{T+1}), P(O|X=(s,a,s'))=e^{r(s, a)}$, and $R=\sum_{(s, a)\in \tau}r(s, a) \Rightarrow
 P(\tau|O)\propto  P(O, \tau)=p(s_1)\prod_{i=1}^T e^{r(s, a)}p(s_{t+1}|s_t, a_t)=p(\tau)e^{R} \propto \mathbf{1}[p(\tau)\neq 0]e^R$ for deterministic environment and fixing $s_1$ by $p(s_1)=\delta(s_1)$. \hza{Why probability $p(a_t|s_t)$ is omitted here? we can only assume a uniform action prior to make SAC holds. Otherwise the entropy should be $D_{KL}(q(a|s)||p(a|s))$ where $p(a|s)$ is the prior action distribution.}
\item Let $\pi(s, a)$ induce the distribution $\hat{p}(\tau)$, we have
$$-D_{KL}(\hat{p}(\tau)||p(\tau|O))=E_{\tau\sim \hat{p}(\tau)}\left[R(\tau)-\sum_{s_t,a_t\in \tau}\log \pi(a_t|s_t)\right]$$
\item In Structured Variational Inference, assume that we use $q(\tau)$ sampled through a policy $\pi(a|s)$ to approx $p(\tau|O)$, then we have  
$$\log p(O_{1:T})=\log \int_\tau p(O, \tau)\frac{q(\tau)}{q(\tau)}d\tau=\log E_{\tau\sim q}\left[p(O,\tau)/q(\tau)\right]\ge E_{\tau\sim q}\left[\log p(O, \tau)-\log q(\tau)\right]$$
$$=E_{\tau\sim q}\left[ \sum_{t=1}^T r(s_t, a_t)-\log \pi(a_t|s_t)\right]$$

by the \href{https://mbernste.github.io/posts/elbo/}{ELBO bound} that $\log p(x)\ge E_{Z\sim q}[\frac{p(x,z)}{q(z)}]=ELBO(x, z, q)$ where $p(x,z)=p(z)p(x|z)$. The reason that we can do this is because we can evaluate $p(O|\tau)$ for $X=O$ and $Z=\tau$, which is the decoder (or the joint distribution easily). \todo{check why we do not normalize p(O|X).}
\item note on the ELBO bound: $\log p(x)-ELBO(x, z, q)=D_{KL}(q(z)||p(z|x)))$
\item VAE is derived by 
$$\log p(x)\ge E_{z\sim q(z|x)}\log p(x|z) + E_{z\sim q(z|x)}\log \frac{p(z)}{q(z|x)}=E_{z\sim q(z|x)}\log p(x|z)-D_{KL}[q(z|x)||p(z)],$$
which could be used to optimize $q(z|x)$ and $p(x|z)$ jointly after knowing $p(z)$ and $p(x)$. In RL as inference, we view sampling $\tau$ as $q(z|x)$ and $p(x|z)$ as the reward.
\item \href{https://arxiv.org/pdf/1606.03476.pdf}{GAIL} In Gail, the objective is $$\min_{\pi} d(\rho_\pi, \rho_E)-H(\pi)=\min_{\pi} -H(\pi) + E_{\pi}\log \frac{D(s, a)}{1-D(s, a)}$$.
\item \href{https://arxiv.org/pdf/1802.06070.pdf}{DIAYN} and \href{https://arxiv.org/pdf/1703.08840.pdf}{InfoGAIL} introduces $Z=(z, \tau)$, fixing $p_{\theta}(z)=p(z)$,  and maximize the reward $-H[Z|S]=q_{\phi}(z|s)$. The ELBO bound becomes \hza{This is wrong actually!}
$$\log p(O_{1:T})\ge E_{z\sim p_{\theta}, \tau\sim \pi_{\theta}(a|s,z)}\left[ \sum_t \log q_{\phi}(z|s_t)-\log p(z) -\log \pi(a_t|s_t, z)\right].$$
Similarly to VAE, the encoder and the decoder could be optimized jointly.
\todo{check it carefully if this formulation is correct ..}


\item It's possible to introduce similar tricks by adding a reward to penalize the discontinuities. We assume that the optimality would not be achieved in the boundary as it's usually not safe and unstable. We also assume that we can soft the environment so that there is no discontinuity. Then given $z$ and $\tau$, we can estimate the scale of expected gradients of the reward/state 
\begin{itemize}
    \item \todo{} verify the force soften strategies in PlasticineLab..
    \item penalize the states that is too far away (large Lipschitz) from the expectation through policy gradients.
    \item switch to policy gradient in that case
    \item Or we can measure the uncertainty of each $z$, if for that $z$ the region is continuous, using gradient descent, otherwise using the policy gradient.
\end{itemize}
\item \todo{Exploration}
\item \todo{Convexity v.s. continuous} It seems that it is easier to build the convexity checker to verify if $f(x)\ge x_0+g_{x_0}^T(x-x_0)$.
    \begin{itemize}
        \item \todo{Cutting plane schema?} Pure local gradient is not able to solve global optimization problem. What we should do is to follow the ellipsoid method such that every time we find an evidence, we reduce the probabilities of a region to be the optimum. 
    \end{itemize}
\end{itemize}





\subsection{An attempt on numerical experiment}
%Notes before: let $X, O$ be two variables and we know $p(X|O)$. Then knowing $p(X)$ is not enough to solve $p(O)$. Considering the case $X=\{0, 1\}$ and $O=\{0, 1\}$. In this case, we only know the ratio of $p_{01}$ and $p_{11}$ and the ratio of $p_{01}+p_{00}$ and $p_{10} + p_{11}$. We also know that the sum of all probability is $1$. Three conditions in total can not solve the original system ..


%Knowing $P(X), P(O), P(X|O)$, we should be able to know $P(O|X)=P(O)P(X|O)/P(X)$.

Let's consider the numerical experiment below
\begin{itemize}
    \item Fixing the start state $s_0$, and let's omit it now.
    \item Consider a distribution generated by $n_z$ modes with Gaussian noise. The reward of a trajectory is proportional to the probability to generate the corresponding trajectories, which is the target $p(\tau|O)$, we also have $p(z|O)$. The generative process is factored as $p(z, \tau|O)=p(O|z)p(\tau|z, O)$. Let $p(z, \tau)=$ the prior distribution of trajectories with standard Gaussian and a uniform random $z$ variable. \todo{design the reward definition ..}
    \item $p(O)p(z, \tau|O)=p(O|z,\tau)p(z,\tau)$ which means that $p(O)$ can not be determined yet.
    \item Then for any trajectory, we can compute reward $p(O|\tau)$ through the Bayesian rule and $p(\tau|z, O)$ easily, thus we can compute the true $p(z|\tau, O)$.
        \begin{itemize}
            \item $\log p(O|z, \tau)=\log p(z, \tau|O) + \log p(O) - \log p(z,\tau)$
            \item reward: $\log p(O|\tau)=\log \left(\sum_z p(z, r|O)\right) +\log p(O) -\log p(\tau)$
            \item $\log p(z|\tau, O)=\log \frac{p(z, \tau,O)}{p(\tau, O)}=\log \frac{p(O|z,\tau)p(z)}{p(O|\tau)}=\log p(z,\tau|O)-\log(\sum_z p(z, r|O))$
            \item To make the reward meaningful (negative), we have $\log p(O) \le \log p(z, \tau) - \log p(z, \tau|O)$ for any $z, \tau$.
            \item We can decompose the reward into two parts $p(O|z, \tau) = e^{R_1(\tau)+R_2(\tau, z)}$.
        \end{itemize}
    \item The goal is to fit a generative model $q(z|O)q(\tau|z, O)$.
    \item \todo{} Notice that $p(\tau, O)=p(\tau|O)p(O)$, we need to verify that for any $q$, the ELBO bound holds that 
    $$\log p(O)\ge E_{z, \tau\sim q} \left[\log p(\tau, z, O) -\log q(z, \tau)\right],$$
    and the lower bound is maximized for $q=p$, for the correct entropy implementation. The gap should be the KL divergence between $q(z, \tau)$ and $p(z, \tau|O)$.
    \item \todo{} for $n_z=1$, this is simply a normal ELBO bound for RL.
    \item $H_q(z|\tau)$ could be estimated based on $q(z|\tau)$. \todo{} check if this coincidents with the learned discriminator.
        \begin{itemize}
            \item 
        \end{itemize}
    \item Compute the loss with the ground truth policy ...
\end{itemize}


\subsection{continuous domain clustering}
\label{sec:VAE_cluster_continuous}
In traditional VAE, for $n_z\rightarrow \infty$, fixing any continuous $q_{\theta}$ function, for any $z$ the generated $q_{\theta}(z|x)$ must be continuous, thus $p_{\phi}(z|X)$ will obviously classify different continuous region with different $z$.

%For VAE, for non-continuous region, if we do not properly split the region, 
To ensure that $q_{\theta}(z|\tau, O)$ favors continuous region, we can use a guassian mixture model on the last layer of the Lipschiz constrained $q_{\theta}$ network. Each $z$ has an embedding, and we assign a probability propotional to the distance of $z$ and the embedding of $\tau$. Thus, when $n_z$ is large enough and the embedding is Lipschiz constrained w.r.t. $r$, we can ensure in each domain there is always a continuous path but we can not make the whole domain continuous. 
%$$\log p(z|\tau, O) = -(f_{\phi}(\tau, O) - e_z)^2$$
%$$\Vert f_{\phi}(\tau_1, O) - f_{\phi}(\tau_2,O)\Vert\le |p(z|\tau_1, O)|^{1/2}+|p(z|\tau_2, O)|^{1/2} \le L\Vert \tau_1 - \tau_2\Vert$$


\section{asymptopic optimality}

Another idea: We need first prove the \href{https://stats.stackexchange.com/questions/256254/universal-approximation-capabilities-of-mixture-models}{the universal approximation capabilities} based on the Gaussian mixture model, and then some similar idea of the \href{https://arxiv.org/pdf/1810.04090.pdf}{convergence of EM}. If we have enough random sample, we can always have a possibility to sample a trajectory around the continuous region of the global optimum -- prove that our algorithm will preserve the global optimum. 

